FLMarket: Enabling Privacy-preserved Pre-training Data Pricing for Federated Learning

Federated Learning (FL), as a mainstream privacy-preserving machine learning paradigm, offers promising solutions for privacy-critical domains such as healthcare and finance. Although extensive efforts have been dedicated from both academia and industry to improve the vanilla FL, little work focuses on the data pricing mechanism. In contrast to the straightforward in/post-training pricing techniques, we study a more difficult problem of pre-training pricing without direct information from the learning process. We propose FLMarket that integrates a two-stage, auction-based pricing mechanism with a security protocol to address the utility-privacy conflict. Through comprehensive experiments, we show that the client selection according to FLMarket can achieve more than 10% higher accuracy in subsequent FL training compared to state-of-the-art methods. In addition, it outperforms the in-training baseline with more than 2% accuracy increase and 3x run-time speedup.

==> abstract.tex <==
\begin{abstract}
Federated learning (FL) has been a popular paradigm, which allows clients to participate in the task without exposing their raw data to the server. 
In an FL data market, the FL task publisher (i.e. server) aims to attract high-quality clients to participate in FL tasks. 
On the other hand, the participating clients aim to maximize their rewards and cover their training costs.
It is crucial for the server and clients to reach a consensus before the training begins. 
Therefore, an effective incentive mechanism in advance of training is non-trivial to make the success of an FL task. 
However, most existing incentive mechanisms rely on the training performance of the clients, thus can only be applied after the training starts. 
In order to design an effective pre-training incentive framework, it requires 
(i) accurately pricing each client based on their true value, thus incentive clients to join the training;
(ii) precisely profiling clients and getting the true value of the clients, without revealing clients' sensitive information.
To address these challenges, we present \projecttitle, an incentivized pre-training incentive framework for FL. 
We design an auction mechanism that interacts with the server and clients to obtain a consensus payment while ensuring truthful pricing for the clients. 
Additionally, we propose a privacy-preserving profiling approach that comprises a novel data score function, and an additive secret-sharing method to help the central server to obtain the true value of each client. 
We evaluated \projecttitle against four state-of-the-art baselines on two applications of three datasets.
Experimental results demonstrate that \projecttitle attains an average accuracy improvement of 11.25\%, and a convergence speed up to 2.92 $\times$ faster than that of the baselines.
\end{abstract}

==> algorithms/algo-baowsrs.tex <==
\begin{algorithm}[t]
  \DontPrintSemicolon
  \SetKwProg{Fn}{}{}{}\SetKwFunction{BWWHS}{BW\_aware\_WHSamp}%
  \Fn(){\BWWHS{$items$, $sampleSize$, $W^{in}$, $C^{in}$}}{
    \tcp{Set to store counts of sampled items for all sub-streams}
    $C^{out} \gets \emptyset$\;
    \tcp{$sample$: set of items sampled within a time interval}
    $sample$ $\gets$ $\emptyset$\;
    \tcp{Update $S$, a set of sub-streams seen so far within the time interval}
    $S$ $\gets$ {\tt Update}($items$)\;
    \tcp{Decide the sample size for each sub-stream}
    $N$ $\gets$ {\tt getSampleSize}({\em sampleSize}, $S$)\;

    \ForAll{$S_{i} \in S$}{ 
      $c_i$ $\gets |S_i|$ \tcp{\em $S_i$: sub-stream i}
      $sample_{i} \gets$ {\tt RS}($S_i$, $N_{i}$) \tcp{Reservoir sampling}
      \tcp{Compute the weight of $sample_{i}$ according to Equation~\ref{eqn:weight}}
      % $w_i$ $\gets$ $1$\;
      \If{$c_i  > N_{i}$}{
        $w_i$ $\gets$ $\frac{c_i}{N_{i}}$\;
        \tcp{update weight for $S_i$}
        $W^{out}_i \gets W^{in}_i * w_i * \frac{C^{in}_i}{c_i}$\; \label{alg:iawhsamp:fix}
        $C^{out}_i \gets N_i$\;
      }
      \Else{
        $W^{out}_i \gets W^{in}_i$\;
        $C^{out}_i \gets c_i$\;
      }
    }
    \Return $sample$, $W^{out}$, $C^{out}$\;
  }

\caption{\bf Interval-agnostic WH sampling}
\label{alg:iawhsamp}
\end{algorithm}

% \begin{algorithm}[t]

% \myfontsize
% \SetLine

% \underline{{\bf {\tt  BW\_aware\_WHSamp}($items$, $sampleSize$, $W^{in}$, $C^{in}$)}}\\
% \Begin{
%     $C^{out} \leftarrow \emptyset$;  {\commentfontsize // {\em Set to store
%         counts of sampled items for all sub-streams}}\\
%     $sample$ $\leftarrow$ $\emptyset$; {\commentfontsize // {\em Set of items
%         sampled within the time interval}}\\
%     {\commentfontsize // {\em S: set of sub-streams seen so far within the time interval}}\\
%     $S$ $\leftarrow$ {\tt Update}($items$); {\commentfontsize // {\em Update the set of sub-streams}}\\
% 	{\commentfontsize // {\em Determine the sample size for each sub-stream}}\\
%     $N$ $\leftarrow$ {\tt getSampleSize}({\em sampleSize}, $S$)\;
   
%     \ForAll{$S_{i} \in S$}{ 
%       $c$ $\leftarrow |S_i|$; {\commentfontsize // {\em $S_i$: sub-stream i}}\\
%       $sample_{i} \leftarrow$ {\tt RS}($S_i$, $N_{i}$);
%       {\commentfontsize // {\em Reservoir sampling }}\\
%       {\commentfontsize // {\em Compute the weight of $sample_{i}$ according to Equation \ref{eqn:weight}}}\\
%       $w$ $\leftarrow$ $1$\;
%       $C^{out}_i \leftarrow c$\;
%       \If{$c$  $>$ $N_{i}$}{
%         $w \leftarrow \frac{c}{N_{i}}$\;
%         $C^{out}_i \leftarrow N_i$\;
%       }
%       $W^{out}_i \leftarrow W^{in}_i * w * \frac{C^{in}_i}{c}$; {\commentfontsize // {\em
%           update weight for sub-stream i}}\\

%     }
%     \Return $sample$, $W^{out}$, $C^{out}$;
% }

% \caption{\bf: Bandwidth aware weighted hierarchical sampling}
% \label{alg:baowsrsAlgo}
% \end{algorithm}

\eat{

{\bf Myungjin's Note: }

\begin{itemize}

\item Each node independently maintains intervals. Intervals are not
  synchronized.

\item $\mathcal{E}_{i,j}$ is a critical path for sub-stream $i$ to node $j$.

\item Let $W_{i,j}$ be a calibrated weight for sub-stream $i$ on node $j$.

\item Let $M_{i,j}$ be the count of items of sub-strem $i$ sent from node $j$ to
  node $j+1$ where $j$ and $j+1$ $\in \mathcal{E}_{i,j+1}$ and node $j+1$ is node
  $j$'s immediate upstream node in the critical path.
\end{itemize}

Node $j$ sends to node $j+1$ a pair of $\{W_{i,j}, M_{i,j}\}$, followed by a
series of items selected from node $j$.

\textbf{1) Ideal case:} $W_{i,j} = W_{i,j-1} * w_{i,j}$ where $w_{i,j} = C_{i,j} /
N_{i,j}$. 

Similar to Equation~\ref{eqn:multsum},
\[
SUM_{i,j} = (\sum_{k=1}^{Y_{i,j}} I_{i,j,k}) \times \prod_{e\in \mathcal{E}_{i,j}} w_{i,e}
\]
That is, $W_{i,j} = \prod_{e\in \mathcal{E}_{i,j}} w_{i,e}$.

\textbf{2) When the number of arrived items at node $j$ is less than the number
  of sampled items at node $j-1$:} $W_{i,j} = W_{i,j-1} * w_{i,j} * f_{i,j}$
where $f_{i,j}$ is a correction factor to readjust the calibrated weight
accureately. 

We want to make sure $SUM_{i,j-1} \simeq SUM_{i,j}$.

\begin{eqnarray}
SUM_{i,j-1} & = & (\sum_{k=1}^{Y_{i,j-1}} I_{i,j-1,k}) * W_{i,j-1} \nonumber \\
& = & (\sum_{k=1}^{Y_{i,j-1}} I_{i,j-1,k}) * \frac{C_{i,0}}{N_{i,j-1}}
\end{eqnarray}

\begin{eqnarray}
SUM_{i,j} &=& (\sum_{k=1}^{Y_{i,j}} I_{i,j,k}) * W_{i,j}  \nonumber \\
  &=& (\sum_{k=1}^{Y_{i,j}} I_{i,j,k}) * W_{i,j-1} * w_{i,j} * f_{i,j}  \nonumber \\
  &=& (\sum_{k=1}^{Y_{i,j}} I_{i,j,k}) * W_{i,j-1} * \frac{C_{i,j}}{N_{i,j}} * f_{i,j}
      \nonumber \\
  &=& (\sum_{k=1}^{Y_{i,j}} I_{i,j,k}) * W_{i,j-2} * \frac{C_{i,j-1}}{N_{i,j-1}}
      * \frac{\alpha N_{i,j-1}}{N_{i,j}} * f_{i,j} \nonumber \\
  &=& (\sum_{k=1}^{Y_{i,j}} I_{i,j,k}) * \frac{\alpha C_{i,0}}{N_{i,j}} * f_{i,j}
\end{eqnarray}

$C_{i,j} = \alpha N_{i,j-1}$ where $0 < \alpha \le 1$.

Since
$(\sum_{k=1}^{Y_{i,j-1}} I_{i,j-1,k}) / N_{i,j-1} \simeq (\sum_{k=1}^{Y_{i,j}}
I_{i,j,k}) / N_{i,j}$,
term $\alpha C_{i,0} * f_{i,j}$ should be equal to $C_{i,0}$, in order to make
$SUM_{i,j-1} \simeq SUM_{i,j}$. Thus, we have $f_{i,j} = 1/\alpha = N_{i,j-1} / C_{i,j}$.


\begin{figure}[t]
\centering
\subfigure[Example topology]{
\includegraphics[width=.45\textwidth]{figuresTex/figs/simpleexp}
\label{fig:exptopo}}
\subfigure[Misaligned interval viewed at Node 2]{
\includegraphics[width=.25\textwidth]{figuresTex/figs/simpleexp2}
\label{fig:misalign}}
\caption{A simple example.}
\label{fig:simpleexp}
\end{figure}

\textbf{Example.} Consider a case in Figure~\ref{fig:simpleexp}. Because
intervals between nodes 1 and 2 are not aligned (see Figure~\ref{fig:misalign}),
a calibrated weight at node 2 should be readjusted. At node 2 in the example,
$\alpha = C_2/N_1$. Hence, $W_2 = W_1 * C_2/N_2 / \alpha = C_0 / N_1 * C_2 / N_2
* N_1 / C_2 = C_0 / N_2$. At node 1, $W_1 = C_0/N_1$. Thus, 

For simplicity, we skip the index number for a sub-stream. Then,
$ SUM_1 = (\sum_{k=1}^{Y_1} I_{1,k}) * C_0/N_1$ and
$ SUM_2 = (\sum_{k=1}^{Y_2} I_{2,k}) * C_0/N_2$. Thus,
$SUM_1 \simeq SUM_2$.

}

==> algorithms/algo-ossolover.tex <==
\begin{algorithm}[t]
  \DontPrintSemicolon
    \KwIn{
  	{
  		\\
  		$R$: a global parameter represents the computing resources\\
  		$U$: a set of osmotic microservice\\
  		$N$: a set of microservice of given application\\
  		$C$: the constraint of network latency 
  	}
  	
  	\KwOut{
  	  \\
  	  $S$: a feasible solution
  	}
  }

  \SetKwProg{Fn}{}{}{}\SetKwFunction{OPT}{BBOpt}%
  \Fn(){\OPT{$U$, $N$, $C$}}{
   {\commentfontsize // {\em Calculate an optimal solution}}\\
  $SOpt$ $\gets$ {\tt Solver}($U$, $N$, $C$, $R$) \\
  \If{{\tt Isfeasible}($SOpt$)}{
  	\Return $SOpt$
  }
  \Else{
  	   $Cons$ $\gets$ $U$, $N$, $C$ \\
  	   {\tt BranchAndBound}($Cons$, $Solutions$, $Selected$, $SOpt$)
  }
  }
  
  \SetKwProg{Fn}{}{}{}\SetKwFunction{BAB}{BranchAndBound}%
  \Fn(){\BAB{$Cons$, $Solutions$, $Selected$, $SOpt$}}{
  
  	  {\commentfontsize // {\em Move the $0$ or $1$ to $S'$ until meet the value which is not $0$ or $1$ value}}\\
  	  $S'$ $\gets$ {\tt MoveValue}($SOpt$)\\
  	   {\commentfontsize // {\em Add $0$ to $S'$, i.e., move to left}}\\
  	   $SLeft$ $\gets$  $S' \cup 0$ \\
  	    {\commentfontsize // {\em Add $1$ to $S'$, i.e., move to right}}\\
  	   $SRight$ $\gets$  $S' \cup 1$ \\
  	   {\commentfontsize // {\em Remove the constraints which links to the $SLeft$}}\\
  	   $U'$, $N'$, $C'$ $\gets$ {\tt ConstraintClean($SLeft$, $Cons$)}\\
  	   $ConsLeft$ $\gets$ $U'$, $N'$, $C'$ \\
  	    {\commentfontsize // {\em Remove the constraints which links to the $SRight$}}\\
  	   $U'$, $N'$, $C'$ $\gets$ {\tt ConstraintClean($SRight$, $Cons$)}\\
  	   $ConsRight$ $\gets$ $U'$, $N'$, $C'$ \\
  	   {\commentfontsize // {\em Calculate an optimal solution}}\\
  	   $SOpt'$ $\gets$ {\tt Solver}($ConsLeft$, $R$) \\
  	    \If{{\tt Isfeasible}($SOpt'$)}{
  	      {\commentfontsize // {\em Combine the inherited solution and the computed solution}}\\
  			$Solu$ $\gets$  $SLeft \cup SOpt'$ \\
  			{\commentfontsize // {\em One solution found}}\\
  			$Solutions$ $\gets$ $solu$ \\
  		}
  		\Else{
  	   	    {\commentfontsize // {\em Add the computed solution and constraints}}\\
  	   	    $Selected$ $\gets$ [$SOpt'$, $ConsLeft$]
  		}
  		
  	   $SOpt'$ $\gets$ {\tt Solver}($ConsRight$, $R$) \\
  	    \If{{\tt Isfeasible}($SOpt'$)}{
  	      {\commentfontsize // {\em Combine the inherited solution and the computed solution}}\\
  			$Solu$ $\gets$  $SRgith \cup SOpt'$ \\
  			{\commentfontsize // {\em One solution found}}\\
  			$Solutions$ $\gets$ $solu$ \\
  		}
  		\Else{
  	   	    {\commentfontsize // {\em Add the computed solution and constraints}}\\
  	   	    $Selected$ $\gets$ [$SOpt'$, $ConsRight$]
  		}
  		\While{$Selected$ $\neq$ $\emptyset$}{
  			$Cons'$, $SOpt'$ $\gets$ {\tt Pop}($Selected$)\\
  			{\commentfontsize // {\em Traversal all solutions through recursion}}\\
  			\BAB{$Cons'$, $Solutions$, $Selected$, $SOpt'$}
  		}
  }

\caption{\bf: B\&B Based Minimization}
\label{alg:osoptimzer}
\end{algorithm}


==> algorithms/algo-overview.tex <==
\begin{algorithm}[t]
\myfontsize
  \DontPrintSemicolon
  %\SetKwInOut{Input}{input}
  %\Input{streaming {\em query} (only for root), {\em  budget}, {\em parent}}
  
  \KwIn{
  	{
  		\\
  		$query$: streaming query (only for root)\\
  		$budget$: resource budget to execute the query \\
  		$parent$: successor node\\
  	}
  }
  \BlankLine

  \Begin{
    \ForEach{time interval} {
      $size$ $\gets$  {\tt  costFunction}($budget$)\; \label{alg:overview_cost}
      {\commentfontsize // {\em $W^{in}$: Weight set from downstream nodes}}\\
      {\commentfontsize // {\em $C^{in}$: Count set from downstream nodes}}\\
      \{$W^{in}$, $C^{in}$, items\} $\gets$  {\tt  getDataStream}($interval$)\; \label{alg:overview_getdata}
		 
      {\commentfontsize // {\em Weighted Hierachical Sampling ($\S$\ref{subsec:whsamp})}}\\
      {\commentfontsize // {\em $W^{out}$: a map of weights of the $sample$}}\\
      {\commentfontsize // {\em $C^{out}$: a map of counts of the $sample$}}\\
      \{$sample$, $W^{out}$, $C^{out}$\} $\gets$ {\tt WHSamp}($items$, $size$, $W^{in}$, $C^{in}$) \label{alg:overview_whsamp}
	
      \If{$parent$ is not empty}{
        {\commentfontsize // {\em (weight, count, sample) to upstream node}}\\
        {\tt Send}($parent$, $W^{out}$, $C^{out}$, $sample$)\; \label{alg:overview_send}
      } \Else {
        {\commentfontsize // {\em Run query as a data-parallel job} \label{alg:overview_run}}\\
        $result$ $\gets$ {\tt  runJob}($query$, $sample$, $W^{out}$)\;

        {\commentfontsize // {\em Estimate error bounds ($\S$\ref{subsec:errEstimation})}}\\
        $error$ $\gets$ {\tt estimateError}($result$)\;
        \textbf{write} $result \pm error$\; \label{alg:overview_write}
      }
    }
  }
\caption{\bf: \projecttitle's algorithm overview}
\label{alg:overviewAlgo}
\end{algorithm}

% \begin{algorithm}[t]

% \myfontsize
% \SetLine

% \textbf{User input}: streaming {\em query} (only for root), {\em  budget},  and
% {\em parent}\\
% % \underline{Perform OWSRS on Cloud (or Root Node)}\\
% \Begin{
%   {\commentfontsize // {\em Computation in sliding window model ($\S$\ref{subsec:system-model})}}\\
%   \ForEach{time interval} {
%     $sampleSize$ $\leftarrow$  {\tt  costFunction}($budget$)\;
%     {\commentfontsize // {\em $W^{in}$: Weight set from downstream edge nodes}}\\
%     \{$W^{in}$, items\} $\leftarrow$  {\tt  getDataStream}($interval$)\;
		 
%     {\commentfontsize // {\em Perform Weighted Hierachical Sampling ($\S$\ref{subsec:oasrs})}}\\
%     {\commentfontsize // {\em $W^{out}$ is a map of weights of the $sample$}}\\
%     $sample$, $W^{out}$ $\leftarrow$  {\tt WHSamp}($items$, $sampleSize$, $W^{in}$)\; 
	
%     \If{$parent$}{
%       {\commentfontsize // {\em send the sample and weight to next upstream edge node}}\\
%       {\tt Send}($parent$, $sample$, $W^{out}$);
%     } \Else {
%       {\commentfontsize // {\em Run query as a data-parallel job to process the sample }}\\
%       $output$ $\leftarrow$ {\tt  runJob}($query$, $sample$, $W^{out}$)\;

%       {\commentfontsize // {\em Estimate the error bounds of query result/output ($\S$\ref{subsec:errEstimation})}}\\
%       $output \pm error$ $\leftarrow$ {\tt estimateError}($output$)\;
%     }
%   }
% }

% \caption{\bf: \projecttitle's algorithm overview}
% \label{alg:overviewAlgo}
% \end{algorithm}


==> algorithms/algo-overview2.tex <==
\begin{algorithm}[t]
\myfontsize
  \DontPrintSemicolon
  %\SetKwInOut{Input}{input}
  %\Input{streaming {\em query} (only for root), {\em  budget}, {\em parent}}
  
  \KwIn{
  	{
  		\\
  		$query$: streaming query (only for root)\\
  		$budget$: resource budget to execute the query \\
  		$parent$: successor node\\
  	}
  }
  \BlankLine

  \Begin{
    \ForEach{interval} {
      $size$ $\gets$  {\tt  costFunction}($budget$)\; \label{alg:overview_cost}
      $\Psi \gets $ {\tt getDataStream}($interval$)\; \label{alg:overview_getstream}
      \While{$\Psi$ is not empty} {
        {\commentfontsize // {\em $W^{in}$: Input weight map for sub-streams}}\\
        \{$W^{in}$, items\} $\gets$ {\tt  getDataSet}($\Psi$)\; \label{alg:overview_getdata}
        {\commentfontsize // {\em Weighted Hierachical Sampling ($\S$\ref{subsec:whsamp})}}\\
        {\commentfontsize // {\em $W^{out}$: a map of weights of the $sample$}}\\
        \{$W^{out}$, $sample$\} $\gets$ {\tt WHSamp}($items$, $size$, $W^{in}$) \label{alg:overview_whsamp}
	
        \If{$parent$ is not empty}{
          {\commentfontsize // {\em (weight, sample) to upstream node}}\\
          {\tt Send}($parent$, $W^{out}$, $sample$)\; \label{alg:overview_send}
        } \Else {
          $\Theta \gets \Theta \cup$\{($W^{out}$, $sample$)\}\; \label{alg:overview_theta}
        }
        $\Psi \gets \Psi \setminus$\{($W^{in}$, items)\}\;
      }
      \If{$parent$ is empty}{
        {\commentfontsize // {\em Run query as a data-parallel job} \label{alg:overview_run}}\\
        $result$ $\gets$ {\tt  runJob}($query$, $\Theta$)\;

        {\commentfontsize // {\em Estimate error bounds ($\S$\ref{subsec:errEstimation})}}\\
        $error$ $\gets$ {\tt estimateError}($result$)\;
        \textbf{write} $result \pm error$\; \label{alg:overview_write}
      }
    }
  }
\caption{\bf: \projecttitle's algorithm overview}
\label{alg:overviewAlgo}
\end{algorithm}

% \begin{algorithm}[t]

% \myfontsize
% \SetLine

% \textbf{User input}: streaming {\em query} (only for root), {\em  budget},  and
% {\em parent}\\
% % \underline{Perform OWSRS on Cloud (or Root Node)}\\
% \Begin{
%   {\commentfontsize // {\em Computation in sliding window model ($\S$\ref{subsec:system-model})}}\\
%   \ForEach{time interval} {
%     $sampleSize$ $\leftarrow$  {\tt  costFunction}($budget$)\;
%     {\commentfontsize // {\em $W^{in}$: Weight set from downstream edge nodes}}\\
%     \{$W^{in}$, items\} $\leftarrow$  {\tt  getDataStream}($interval$)\;
		 
%     {\commentfontsize // {\em Perform Weighted Hierachical Sampling ($\S$\ref{subsec:oasrs})}}\\
%     {\commentfontsize // {\em $W^{out}$ is a map of weights of the $sample$}}\\
%     $sample$, $W^{out}$ $\leftarrow$  {\tt WHSamp}($items$, $sampleSize$, $W^{in}$)\; 
	
%     \If{$parent$}{
%       {\commentfontsize // {\em send the sample and weight to next upstream edge node}}\\
%       {\tt Send}($parent$, $sample$, $W^{out}$);
%     } \Else {
%       {\commentfontsize // {\em Run query as a data-parallel job to process the sample }}\\
%       $output$ $\leftarrow$ {\tt  runJob}($query$, $sample$, $W^{out}$)\;

%       {\commentfontsize // {\em Estimate the error bounds of query result/output ($\S$\ref{subsec:errEstimation})}}\\
%       $output \pm error$ $\leftarrow$ {\tt estimateError}($output$)\;
%     }
%   }
% }

% \caption{\bf: \projecttitle's algorithm overview}
% \label{alg:overviewAlgo}
% \end{algorithm}


==> algorithms/algo-owsrs2.tex <==
\begin{algorithm}[t]
\myfontsize
  \DontPrintSemicolon
  
    \KwIn{
  	{
  		\\
  		$items$: input data items\\
  		$sampleSize$: size of sample\\
  		$W^{in}$: weight map from downstream nodes\\
  	}
  }

  \SetKwProg{Fn}{}{}{}\SetKwFunction{WHS}{WHSamp}%
  \Fn(){\WHS{$items$, $sampleSize$, $W^{in}$}}{
     {\commentfontsize // {\em $sample$: set of items sampled within a time interval}}\\
    $sample$ $\gets$ $\emptyset$\; \label{alg:whsamp_sample}
     {\commentfontsize // {\em Update $S$, a set of sub-streams seen so far within the interval}}\\
    $S$ $\gets$ {\tt Update}($items$)\; \label{alg:whsamp_update}
     {\commentfontsize // {\em Decide the sample size for each sub-stream}}\\
    $N$ $\gets$ {\tt getSampleSize}({\em sampleSize}, $S$)\; \label{alg:whsamp_getsize}
    
    \ForAll{$S_{i} \in S$}{ 
      $c_i$ $\gets |S_i|$  {\commentfontsize // {\em \em $S_i$: sub-stream i}}\\
      $sample_{i} \gets$ {\tt RS}($S_i$, $N_{i}$)  {\commentfontsize // {\em Reservoir sampling} \label{alg:whsamp_rs}}\\
       {\commentfontsize // {\em Compute the weight of $sample_{i}$ according to Equation~\ref{eqn:weight}}}\\
      % $w_i$ $\gets$ $1$\; \label{alg:whsamp_wstart}

      \If{$c_i$  $>$ $N_{i}$}{\label{alg:whsamp_wstart}
        $w_i$ $\gets$ $\frac{c_i}{N_{i}}$\;
        $W^{out}_i \gets W^{in}_i * w_i$  {\commentfontsize // {\em update weight of $S_i$} \label{alg:whsamp_need_fix}}\\
      }
      \Else{
        $W^{out}_i \gets W^{in}_i$\; \label{alg:whsamp_noup}
      } \label{alg:whsamp_wend}
    }
    \Return $W^{out}$, $sample$\; \label{alg:whsamp_return}
  }

\caption{\bf: Weighted hierarchical sampling}
\label{alg:whsamp}
\end{algorithm}

% \begin{algorithm}[t]

% \myfontsize
% \SetLine

% \underline{{\bf {\tt  WHSamp}($items$, $sampleSize$, $W^{in}$)}}\\
% \Begin{
%     $sample$ $\leftarrow$ $\emptyset$; {\commentfontsize // {\em Set of items
%         sampled within the time interval}}\\
%     {\commentfontsize // {\em S: set of sub-streams seen so far within the time interval}}\\
%     $S$ $\leftarrow$ {\tt Update}($items$); {\commentfontsize // {\em Update the set of sub-streams}}\\
% 	{\commentfontsize // {\em Determine the sample size for each sub-stream}}\\
%     $N$ $\leftarrow$ {\tt getSampleSize}({\em sampleSize}, $S$)\;
   
%     \ForAll{$S_{i} \in S$}{ 
%       $C_{i}$ $\leftarrow |S_i|$; {\commentfontsize // {\em $S_i$: sub-stream i}}\\
%       $sample_{i} \leftarrow$ {\tt RS}($S_i$, $N_{i}$);
%       {\commentfontsize // {\em Reservoir sampling }}\\
%       {\commentfontsize // {\em Compute the weight of $sample_{i}$ according to Equation \ref{eqn:weight}}}\\
%       $w$ $\leftarrow$ $1$\;
%       \If{$C_{i}$  $>$ $N_{i}$}{
%         $w$ $\leftarrow$ $\frac{C_{i}}{N_{i}}$\;
%       }
%       $W^{out}_i \leftarrow W^{in}_i * w$; {\commentfontsize // {\em update weight for sub-stream i}}\\
%     }
%     \Return $sample$, $W^{out}$;
% }

% \caption{\bf: Weighted hierarchical sampling}
% \label{alg:owsrsAlgo}
% \end{algorithm}

==> algorithms/bin_demo_alg.tex <==
\begin{algorithm}[t]
  \DontPrintSemicolon
  \small  
    \KwIn{
  	{
  	
  		Initial point $\be_{0}$ at which $T$ is differentiable, closed unit ball $\mathbb{B}$, maximum step $N$.
  		
  		initial sampling radius $\epsilon_{0} > 0$, sample radius reduction factor $\theta_{\epsilon} \in [0,1]$, sample size $m \geq K + 1$.
  		
  		Optimality tolerance $\nu_{j} \geq 0$. 
  		Optimality tolerance reduction factor $\theta_{\nu} \in [0,1]$
  		
  	weak wolfe line search parameter $w_1$, $w_2$,  constraints $\mathcal{Q}$
  	}
  	\\
  	\For{$j \in N$}
  	{
  	\textbf{Step 0: Gradient Sampling}
  	
  	Independently sample $\{\be_{j,1}, \be_{j,2}, ..., \be_{j,m}\}$ from $\mathbb{B}(\be_{j}, \epsilon_{j})$;

  	\textbf{Step 1: Search direction calculation}
  	
  	Compute $\bg_{j}$ as the solution of $\arg\min_{g \in \mathcal{G}} ||g||_{2}^{2}$, where $\mathcal{G} = \mathrm{Conv}\{\nabla T(\be_{j,0}), \nabla T(\be_{j,1}), ..., \nabla T(\be_{j,m}) \}$;
  	 
  	\eIf{$||\bg_{j}|| \leq \nu_{j}$}
  	 {$t_{j}$ = 0, set $\nu_{j+1}$ = $\theta_{\nu}\nu_{j}$, $\epsilon_{j+1} $= $\theta_{\epsilon}\epsilon_{j}$;
  	 
  	 \textbf{go to step 3}
  	 }{
  	  set $\nu_{j+1}$ = $\nu_{j}$, $\epsilon_{j+1}$ = $\epsilon_{j}$;
  	  
  	 \textbf{go to step 2}
  	 }
  	
  	\\
  %\zy{EDIT THIS BACK TO NORMAL LINE SEARCH}
  	\\
  	\textbf{Step 2: Step length calculation}
  	\\
  	$\eta_{j} $ = line\_search$(\be_{j,0}, \bg_{j}, w_1, w_2)$
  	\\
  	\textbf{Step 3: Update }
  	$y_{j+1}$ = $\be_{j} - \eta_{j}  \bg_{j}$
  	
  	\eIf{$y_{j+1} \notin \mathcal{Q}$}
  		{
  		\textbf{go to step 4};
  		}
  		{
  		set $\nu_{j+1}$ = $\theta_{\nu}\nu_{j}$, $\epsilon_{j+1} $= $\theta_{\epsilon}\epsilon_{j}$;
  		
  		\textbf{continue}
  		}	
  	\\
  	\textbf{Step 4: Projection}
$\be_{j+1} = \arg\min_{x \in \mathcal{Q}} \frac{1}{2} ||x-y_{j+1}||_{2}^{2}$
  	}
  }
\caption{\bf Projected Gradient Sampling for Video Analytic Offloading  (PGS-VAO)}
\label{alg:PGS}
  \vspace{-1mm}
\end{algorithm}

==> algorithms/hhz_alg.tex <==
% \begin{algorithm}[t]
% \caption{Federated Learning Algorithm IPA}\label{alg:IPA}
% \textbf{Input:}
% client $e \in E = [1,2,...,E]$ \\
% \textbf{Output:}
% global model parameter $w(t)$ \\
% Clients $e$ compute \textbf{Algorithm 2:}ASS-GAD \\
% Server set evaluation function $\mathcal{U}_{e} $ and send it to clients \\
% \For{client $e$ in parallel}
% {
%     Count the local class distribution vector $N_e$. \\
%     Compute Score $s_{e} = \mathcal{U}_{e}(N_e)$, and send $s_{e}$ to Server. \\
% }
% \For{Server}
% {
%     Sort $s_{e}$ and select high score edge clients $k \in K_{s}$. \\
%     Send task to the selected edge clients $k \in K_{s}$. \\
% }
% Set parameters of selected clients $w_{i}(0) = w(0)$ \\
% \For{each round $t = 1,2,... $}
% {
%     \For{each client $k \in K_{s}$ in parallel}
%     {
%         $w_{t+1}^{k} = Client.Train(k, w_{t})$ \\
%     }
%     \eIf{$w_{t+1}^{k}$ pass the client validation}
%     {
%         \textbf{continue} \\
%     }
%     {
%         Remove $k$ from $K_{s}$, and add next high score client into $K_{s}$.
%     }
%     $w_{t+1} = \sum_{k=1}^{K_{s}} \frac{n_{k}}{n}w_{t+1}^{k} \quad$
% }
% \end{algorithm}

% \begin{algorithm}[t]
% \caption{ASS-GAD}\label{alg:ASSGAD}
% \textbf{Initialize:}
% client $e \in E$ count the local class distribution vector $N_e$ \\

% \For{client $e$ in parallel}
% {
%     Randomly divide $N_e$ into $E$ parts, marked $[N_e(1),N_e(2)...N_e(E)]$ \\
%     Send $(E-1)$ parts to each other $(E-1)$ clients while keeping one part locally. \\
%     \eIf{Finish receiving $(E-1)$ parts of each other $(E-1)$ clients}
%     {
%         $N_e'=sum[N_1(e),N_2(e)...N_E(e)]$\\
%         Send $N_e'$ to Server
%     }
%     {
%         \textbf{continue}
%     }
% }
% \For{Server}
% {
%     $N=sum(N_1',N_2'...N_E')$
% }
% \textbf{return $N$}
% \end{algorithm}

==> auction.tex <==

\section{Data marketplace pricing Framework for federated learning}
\label{sec:ipp}

% In this section, we provide an overview of \projecttitle, the design of the data function, the detailed formulation of the auction mechanism, and the algorithms for selecting and pricing the clients.
% We also analyze the truthful property of the proposed top-K client selection and pricing algorithm,
% which means each client is assigned a critical price and can not increase its bid while still being selected by the server~\cite{yang2012crowdsourcing}.
%In this section, we introduce the \projecttitle pricing framework for incentivizing users to share their data for FL training, and then outline some basic properties that our framework must satisfy. 

\di{In this section, we first provide an overview of our pricing framework and how it operates within the FL data market (Section~\ref{subsec:overview}). Then, we present the details of our two-round pricing mechanism, starting from the initial pricing for individual clients (Section~\ref{subsec:first-round}) and following the determination of final price through the second-round multi-client bidding (Section~\ref{subsec:second-round}).}

% We summarize the notations used throughout this paper in Table 1.

% In this section, we first analyze the impact of data quantity and data rarity. Based on that we propose a new data valuation function for data evaluation and we design a pricing function for a single client depending on it (section~\ref{sec:data_evaluation}). 
% Then we formulate a multi-client bidding mechanism for select top-K clients and determine the payment (section \ref{sec:auctiondefinition}). Finally, the truthful property of our mechanism has been analyzed.

\begin{figure}[t]
 \vspace{0mm}
     \centering
    \includegraphics[width=0.48\textwidth]{./figuresTex/figs/framework.pdf}
     \vspace{-6mm}
     \caption{\projecttitle high-level system overview}
     \label{fig:framework}
     \vspace{-6mm}
 \end{figure}

% Furthermore, we select top-K clients and price them (section \ref{subsec:selectandprice}). Finally, the truthful property of our algorithm has been analyzed (section~\ref{sec:truthful}).
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.47\textwidth]{figuresTex/figs/system.pdf}
% \vspace{-3mm}
%  %\caption{\projecttitle's High-level System Overview}
%  \caption{\projecttitle's auction process}
% \label{fig:IPP_framework}
% \vspace{-3mm}
% \end{figure}

% \subsection{Overview of \projecttitle}
% \label{sec:ippoverview}

% Figure~\ref{fig:IPP_framework} shows \projecttitle's auction process, which consists of a \textit{Client profiler} and \textit{Client Selector \& pricer}. 
% We designate the server $S$ as the task publisher in the FL data marketplace and the clients $\mathbb{E}$ as bidders who follow the 4 steps outlined below.
% \begin{enumerate}
%     \item \textit{Task Publication and Bidding:} 
%     The FL task publisher (i.e. server $S$) publishes the task requirements (data, labels, and hardware requirements) 
%     % as well as the total number of anticipated clients $E$ for an FL task $\mathbb{T}$. 
%     A client $e$ who is willing to join the training task submits a bid, i.e., a quoted price for contributing to the model training.
%     Note that, at the end of the auction, only $K$ clients are able to join the task.

%     \item \textit{Client Profiling:} 
%     % The \textit{Client Profiler} interacts with the clients to acquire knowledge regarding global data distributions, in an attempt to precisely profile each client and select high-quality clients.
%     % In this process, the server sends a data score function to all clients and collects the data scores from them (Section \ref{sec:data_evaluation}).
%     The \textit{Client Profiler} interacts with the clients to acquire knowledge about each client's data quality. 
%     In this process, the server sends a data score function to all clients and collects the data scores from them, which reflect the data quality. (Section \ref{sec:data_evaluation}).

%     \item \textit{Client Selection and Pricing:} 
%     After collecting the scores, the \textit{Client Selector \& Pricer} calculates the utility of each client $e$ based on the scores and bids obtained in the previous steps. 
%     The server then selects the top-K clients and determines the payment (Section \ref{subsec:selectandprice}) for the selected clients, which is calculated as its critical price to support truthfulness (Section \ref{sec:truthful}).
%     % \bin{
%     % It also computes the payments for each clients based on XXXX.
%     % }
    
%     \item \textit{Announcement:} 
%     Finally, the server will announce the decisions of the top-K winners as well as the corresponding payments of all selected clients.
%     The whole client selection process is thus complete prior to the training begins. 
% \end{enumerate}  

\subsection{High-level system overview}
\label{subsec:overview}
Our framework involves three parties: the \textit{Data market} (Server), \textit{Data sellers} (Clients) and \textit{Data buyers}. A buyer publishes a FL training task with a budget and the data market groups a set of clients to perform the training task. Finally, the data market returns a trained deep-learning model for the buyer. Figure~\ref{fig:framework} illustrates the high-level system overview of the \projecttitle pricing framework.

\myparagraph{Pipeline}
The whole process for pricing a single client is divided into the following 3 steps.
First, we evaluate data for each client by aggregating and getting global data distribution $N$ with a privacy-aware secret-sharing (PASS) mechanism (see \S \ref{sec:system}).
Then, both $N$ and $\mathcal{U} (N, n_e^c)$ will be sent to the clients, where the clients compute the data score $u_e$ with $n_e^c$ and $N$ altogether.
Finally, all $\{u_e\}_{\forall e \in E}$ will be sent back to the server for pricing the data for each client $e$. 
The clients that contain rarer class data and sufficient data volume will have higher pricing and are regarded as high-quality clients.

\myparagraph{Framework} A seller first needs to make a registration if it is interested in participating in the FL task $\mathbb{T}$(step \textcircled{1}). Thereafter, the data market evaluates the data value that will be shared by each client $e$ and returns an assessed price $ u_e^T$(step \textcircled{2} \S \ref{subsec:first-round}). 
Then, the client $e$ will make a bid (quote) $b_e$ for contributing its data and computing resources (step \textcircled{3} \S \ref{subsec:second-round}). Finally, the data market will determine the final price $p_e^T$ for the clients selected for $\mathbb{T}$ (step \textcircled{4} \S \ref{subsec:second-round}).


%\myparagraph{Privacy leakage}
\di{\myparagraph{Privacy concern}}
We consider a scenario where the model is securely trained using data from both a fully trustworthy party and a party that is honest-but-curious~\cite{}\di{need a reference here}. In this realistic context, the honest-but-curious adversary assumes that the malicious entity will (1) refrain from modifying its own data, as doing so might compromise the model's performance and, if discovered, could damage the trust established with the other participant, and (2) not tamper with the machine learning code. Both parties might desire to review the code executed on the data to guarantee its integrity and security.

In step \textcircled{2} and \textcircled{4}, the global data distribution $N$ is required to help assess a client's price $ u_e^T$ and the final $p_e^T$. Obtaining $N$ may cause the users' personal information leakage as illustrated following. 
The most efficient method is for all clients to share their local data distributions to the server directly. 
However, it exposes the client's data class and the corresponding quantities to both the server and other clients. 
Have data class and quantity are the sensitive information that can infer what the precise ratio of attribute values is (e.g., 90\% females vs. 70\% females)~\cite{zhang2021leakage}, individual habits (e.g., frequently purchased food)~\cite{deshpande2004item}, \lei{Merchandise sales (e.g., most popular products)~\cite{hartmann2023distribution}, population’s financial status (e.g., proportion of people with different levels of income)~\cite{chen2023protecting}}.



% Moreover, exposing the data distribution would impact the effectiveness of the bidding mechanism. When all clients know the data distribution of each other, they can compute the score $u_e$ of others according to Equation~\ref{eq:evaluation function}. Then in bidding phase ($\S$~\ref{sec:auctiondefinition}), the bids submitted by clients may affected by the score of others rather than themselves. It would undermine the fairness of the bidding mechanism.





\subsection{Single Client Price Assessment}
\label{subsec:first-round}
%\lei{Prior to introducing the price assessment mechanism, this subsection conducts an analysis of the pivotal factors influencing data quality. Guided by these identified factors, we formulate a data quality evaluation function capable of ascertaining the pricing for registered clients.}
\di{Pricing a individual client data before training is challenging since it is difficult to have an explicit expression to directly determine the pricing for the data. We break down the data pricing process into two steps. Firstly, how to evaluate individual client data by scoring, where the score should be a reasonable assessment of the impact of client data on subsequent FL training. However, the score itself can only reflect a relative quality of client data and does not represent an actual price. Secondly, we transform the scores of clients into a reasonable actual prices by considering the budget of the data buyers.}

\begin{figure}[h]
\vspace{-3mm}
\centering
    \subfloat[Data quantity]{
    \includegraphics[height=.18\textwidth]{./figuresTex/figs/Amountandacc.pdf}
    \label{fig:Amountandacc}}
    \subfloat[Data balance]{
    \includegraphics[height=.18\textwidth]{./figuresTex/figs/motivation_data.pdf}
    \label{fig:motivation_data}}
    %\subfloat[Free rider attack]{
    %\includegraphics[width=.28\textwidth,height=0.192\textwidth]{./figuresTex/figs/motivation_fake.pdf}
    %\label{fig:motivation_fake}}
    \vspace{-3mm}
    %\caption{The Impact of Data Quantity and Distribution for Training
    %an FL Training Task.}
     \caption{The impact of data quantity and distribution for training
     an FL training task.}
    \label{fig:dsads}
    \vspace{-3mm}
\end{figure}

\myparagraph{Design principles}
\textit{Impact of data quantity and rarity.} According to current research~\cite{deng2021auction,saha2022data,li2021sample}, there are two factors that impact model training accuracy. One is data quantity and another is data rarity. 
For data quantity, when few data are available during the training process, a slight increase in data quantity could significantly improve the training accuracy. 
As more data are added to the training set, the newly added data contribute less to performance gain. 
Therefore, the valuation should be positively correlated to the quantity of data with a diminishing trend of marginal accuracy.

Data used for traditional centralized machine learning is generally evenly distributed, i.e. the number of each class is the same. In FL, evenly distribution of global data can improve the learning performance significantly~\cite{deng2021auction,li2021sample} and we named this distribution as balance distribution in this paper. 
Thus, the evaluation should encourage achieving a global balance across all classes. That means we need more rarity class data to join the FL task to achieve the relative optimal balance.
We also experimentally verify the impact of data quantity and rarity on FL in Appendix~\ref{sec:impact}.

We experimentally investigate the impact of two factors of data, i.e. quantity and distribution, by following experiments where we trained a popular ResNet-56~\cite{he2016deep} model using CIFAR-10~\cite{krizhevsky2012imagenet} dataset in a classical FL setting~\cite{mcmahan2017communication}.

\textit{The value of the client should be positively correlated to the size of data with a diminishing trend of marginal accuracy.}
To investigate the impact of data quantity, we examine the test accuracy of global models that are trained upon different volumes of data. Figure~\ref{fig:Amountandacc} shows the curve of test accuracy against the volume of data and bars of $\Delta Accuracy$ for every 1,000 incremental data. 
From the results, we could observe that the test accuracy increases with the increase in the amount of training data. However, the $\Delta Accuracy$ decreases rapidly, indicating that the marginal contribution of data to the test accuracy is limited when the data size is large.

\textit{The evaluation should encourage achieving a global balance across all classes.}
To evaluate the impact of data distribution, we compare the model accuracy under three distributions. 
(i) The data distributions are balanced across classes both locally for each client and globally for the server, namely \textit{local balance and global balance}. 
(ii) The data distribution is imbalanced locally but balanced globally, namely \textit{local imbalance and global balance}. 
(iii) The data distributions are both locally and globally imbalanced, namely \textit{local imbalance and global imbalance}.
Figure~\ref{fig:motivation_data} shows that the data imbalance significantly deteriorates the learning performance of FL training. 
However, when the global data is balanced while the local data is still imbalanced (the green curve in Figure~\ref{fig:motivation_data}), the accuracy degradation for FL training is much milder. In the practical scenario, the data distribution of local data is determined by the characteristics of end users, and hence cannot be controlled by the central server. Fortunately, the global distribution could be adjusted in the client evaluation process to mitigate the issue of local data imbalance.

\myparagraph{Score function}
Based on the observed two factors, we proposed a new data evaluation function $\mathcal{U}$ as follows.
\begin{equation}
\label{eq:evaluation function}
    \mathcal{U}(N,n_e^c) =\sum_{c=1}^{C} \phi(n_{e}^{c})\cdot \theta_{c} (N)
\end{equation}
Where $N$ is the global data distribution that indicates the data volume of the classes from all registered clients, and $n_e^c$ denotes the data volume of class $c$ in client $e$. $\mathcal{U}(N,n_e^c)$ sums up the evaluation scores of individual data samples across all classes, i.e.,$\phi(n_{e}^{c})\cdot \theta_{c} (N)$. 

% Let $n^{c}$ denotes the total number of data for class $c$, i.e. $ N = [n^{1}, n^{2} ... n^{C} ]$ and $\sum_{c=1}^{C} n^{c} = n$, we sums up data score of each class $c$ as client's data score. The class data score function $\mathcal{V}$ is defined as follows.
The two coefficients $\phi(n_{e}^{c})$, $\theta_{c}(N)$ in Equation \ref{eq:evaluation function} represent the effect of data quantity and class rarity respectively.  
% Data score is affected by two things: data quantity and data rarity. Then the class data score function $\mathcal{V} (N, n_e^c)$ considering two coefficients:
1) data quantity coefficient $\phi(n_{e}^{c})$, on the other hand, is a specific coefficient that gives the value based on data samples $n_e^{c}$ belonging to class $c$.
2) class rarity coefficient $\theta_{c} (N)$ is a generic coefficient with respect to global data distribution $N$ and calculates the rarity of each class $c$ from $N$.  
The following illustrates the details of two coefficients.


\textit{Data Quantity Coefficient}
% Our observation of the effect of model accuracy with the amount of data shows that the effect of data volume on accuracy is progressively reduced, thus we model this effect as a function of the integral of $-lnx$ over the interval [0-1].
We model the quantity effect as a function of the integral of $-lnx$ over the interval [0-1]. 
That can simulate the effect of positively correlated to data quantity with a diminishing trend of marginal contribution.
The quantity coefficient for individual class $c$ is defined as: 
\begin{equation}
    \phi(n_{e}^{c}) = \int_{0}^{r_e^c} -lnx dx
\label{eq:quantity_coe}
\end{equation}
 
We set $r_e^c$ as the upper limit of integration for the function, and $r_e^c$ is a normalized value of $n_e^c$ to set all $\phi(n_e^c)$ to the same scale. 
We assume that when $n_{e}^{c} \geq n / (E, C)$, any class that contains more than the average number of data will not receive a further reward. Thus we define the max value of $r_e^c$ as 1. When the data volume of class $c$ on client $e$ is greater than $\frac{n}{E\cdot C}$, $r_e^c=1$.
\begin{equation}
    % r_e^c = \min \{ \frac{n_{e}^{c}}{n/ (E \cdot C)} , 1\} 
r_e^c =\left\{\begin{matrix}
\frac{n_{e}^{c}}{n/ (E \cdot C)}, n_e^c<\frac{n}{E\cdot C}\\ 
1,n_e^c\geq\frac{n}{E\cdot C}
\end{matrix}\right.
\end{equation}

% \myparagraph{The importance of modeling Data Quantity in Granularity}
% Figure~\ref{fig:Amountandacc} shows that the data quantity is highly correlated with the final training accuracy.
% When few data are available during the training process, a slight increase in data quantity could significantly improve the training accuracy.
% As more data are added to the training set, the newly added data contribute less to performance gain. 
% Thus we model this non-linear relation between the data quantity and the training accuracy with data quantity coefficient $\phi(n_{e}^{c})$ (i.e., Equation~\ref{eq:quantity_coe}) to denote the importance of each individual data sample. 

\textit{Data Rarity Coefficient}
The data quantity coefficient assumes equality importance for samples across different classes. However, valuing more rare classes helps to improve the uniformity of final global data distribution. 
The rarity of the class $c$ data is defined by $\theta_{c}$:
\begin{equation}
 \theta_{c} (N) =  1 - n^{c} / n
\end{equation}
$n^{c}$ is the total number of data for class $c$ and $n$ is the total number of data in $N$.
We use min-max normalization \cite{friedman2019assessment} to normalize $\theta_{c}(N)$ for $\forall   n^{c} \in N$ and rescale it such that $ \theta_{c}(N) \in [\min\{{N}\}, \max{\{N}\}]$.
% We also validate the necessity of $\theta_{c}(N)$ in Section \ref{sec:sen_analysis} and Figure~\ref{fig:test_theta}.

\myparagraph{Translate the score to a price}
The server will obtain a score $u_e$ from the client $e$ using the evaluation function proposed above. 
This score can be used for ranking and comparing the quality of client data. However, it is not a meaningful value for pricing the data of the client. 
Then we propose the use of a conversion function to transform the score $u_e$ to a meaningful price $u_e^T$ using the following equation:

% \begin{equation}
%     u_e^T = \frac{R}{K} * \frac{u_e}{\sum_{e \in \mathbb{E}} u_e} * K
%     \label{eq:utilityfunction}
% \end{equation}
% where $\frac{R}{K}$ is the average reward given that $K$ clients are finally selected and $\frac{u_e}{\sum_{e \in \mathbb{E}} u_e} * K$ is the probability of client $e$ be selected.
\begin{equation}
\label{eq:single pricing}
% \label{eq:utilityfunction}
    % u_e^T = \frac{R}{K} * \frac{E}{\sum_{e \in \mathbb{E}} u_e} * u_e
    u_e^T = R * \frac{u_e}{\sum_{e \in \mathbb{E}} u_e}
\end{equation}
% where $\frac{R}{E}$ is the average reward given that $K$ clients are finally selected and $\frac{E}{\sum_{e \in \mathbb{E}} u_e} * u_e$ can be interpreted as the scale factor for client $e$ according to its score and the average score for all clients $\mathbb{E}$.
\lei{The function divides the budget according to the value of the data score to determine the price $u_e^T$ .}


% \subsection{Pre-Training Auction in \projecttitle}
\subsection{Multi-client Bidding}
\label{subsec:second-round}
According to the pricing for the single client above, we formulate a multi-client bidding mechanism for client selection. 
% According to the evaluation of the data presented above, we formulate the auction mechanism for client selection.

\myparagraph{Bidding mechanism}
\emph{Bidding Entity:}
We follow the design of a classical bidding mechanism, where the server $S$, as a task publisher in an FL data marketplace, orchestrates the bidding procedures. 
\lei{The server $S$ get an FL task $\mathbb{T}$ with an estimated budget $R$ from the buyer and publish it to the clients.} 
A client pool $\mathbb{E}$, composed of $E$ clients, is the set of all potential candidates for FL task $\mathbb{T}$. 
The bidding procedures aim to select the most valuable $K$ clients who will join the FL task $\mathbb{T}$ and get payments from $S$.

\emph{Bid Information:}
\lei{When received the task information from the server $S$, each client $e$ prepares the data which fits the task.
The client $e$ also asks for evaluation an pricing for their data by the server. 
After evaluating the data, each client $e$ will get a score for its data and send it to the server for pricing. The server combines the scores of all the clients to price each client and sends the price $u_e^T$ to the corresponding client $e$.
Client $e$ makes a bid based on the price $u_e^T$.}
Particularly, a bid includes the quoted price and statistics of data volume and distribution for each client $e$.
We denote the bid from client $e$ as $b_e$ and the set of bids of $E$ clients is $\mathbb{B} = \{b_e\}_{e \in \mathbb{E}}$. To simplify the notation, we also use $b_e$ to represent the payments required by client $e$ in its bid when we calculate the utility values of each client.

\emph{Server-side Utility Function:}
\lei{After the sever receives the bids $\mathbb{B}$ from clients}. 
We further define the utility of the client $e$ as the quotient of $b_e$ and $u_e^T$, which indicates\lei{ the markup ratio of bid price over the assessed value of their data}
Finally, we calculate the utility value $v_e$ for client $e$ as below.
\begin{equation}
    v_e = b_e / u_e^T
\end{equation}
In addition, the set of the utility values for all clients $\mathbb{E}$ is $\mathbb{V} = \{v_e\}_{e \in \mathbb{E}}$. \lei{Note that for a rational client,}
% After aggregating global data distribution from all clients, the server $S$ distributes a data evaluation function to each client $e$ to compute the score (value) of data contributed by each $e$ (Section \ref{sec:data_evaluation}). 

% the server will get a score of each client $e$ denote as $u_e$.
% $\mathbb{U}$ stands for the set of all scores for $\mathbb{E}$. 
% These scores can be used for ranking and comparing the quality of client data. However, it is not a meaningful value for pricing the data of the client. 
% We propose the use of a conversion function to transform the score $u_e$ to a value that can be compared to $b_e$ using the following equation:

% \begin{equation}
%     u_e^T = \frac{R}{K} * \frac{E}{\sum_{e \in \mathbb{E}} u_e} * u_e
%     % u_e^T = \frac{R}{K} * \frac{u_e}{\frac{\sum_{e \in \mathbb{E}} u_e}{E}}
%     \label{eq:utilityfunction}
% \end{equation}
% where $\frac{R}{K}$ is the average reward given that $K$ clients are finally selected and $\frac{E}{\sum_{e \in \mathbb{E}} u_e} * u_e$ can be interpreted as the scale factor for client $e$ according to its score and the average score for all clients $\mathbb{E}$.


% \begin{algorithm}[t]
%     \caption{Top-K Selection and Pricing in \projecttitle}
%     \label{algorithm1}
%     \textbf{Input:} Bids $\mathbb{B} = \{b_e\}_{e \in \mathbb{E}}$ and Scores $\mathbb{U^T} = \{u_e^T\}_{e \in \mathbb{E}}$\\
%     \textbf{Output:} Decisions $\mathbb{D} = \{d_e\}_{e \in \mathbb{E}}$ and Prices $\mathbb{P} = \{p_e\}_{e \in \mathbb{E}}$\\
%     // Top-K winners selection\\
%     \For{each $e \in \mathbb{E}$}{
%         $d_e = 0$ \\
%         $p_e = 0$ \\
%         $v_e = u_e^T - b_e$ {\color{teal} \raggedright \footnotesize{\null\hfill Calculate the utility value}}\\ 
%     }
%     $\mathbb{S} \leftarrow argsort(\mathbb{V},K)$  {\color{teal} \raggedright \footnotesize{\null\hfill Return the indices of top-K values}}\\ 
%     $I_{K+1} \leftarrow argmax(\mathbb{V},K+1)$ {\color{teal} \raggedright \footnotesize{\null\hfill Return the index of the $K+1$-th maximum value}}\\ 
%     \For{each $e \in \mathbb{E}$}{
%         \If{$e \in \mathbb{S}$}{
%             $d_e = 1$\\
%         }
%         \Else{
%             $d_e = 0$\\
%         }
%     }
%     // Price determination\\
%     \For{each $e \in \mathbb{E}$}{
%         \If{$e \in \mathbb{S}$}{
%             \If{$v_e > 0$}{
%                 $\delta_e = v_e - v_{I_{K+1}}$ {\color{teal} \raggedright \footnotesize{\null\hfill Calculate the utility difference between $e$ and $I_{K+1}$.}}\\ 
%                 $p_e = b_e + \delta_e$
%             }
%             \Else{
%                 $p_e = u_e^T$
%             }
%         }
%     }
% \Return{$\mathbb{D}$ and $\mathbb{P}$}
% \end{algorithm}



% \myparagraph{Selection and Pricing}
% According to $\mathbb{V} = \{v_e\}_{e \in \mathbb{E}}$, the server $S$ selects a top-K winners from $\mathbb{E}$, 
% % We denote decisions for all client as $\mathbb{D} = \{d_e\}_{e \in \mathbb{E}}$. 
% % Particularly, $d_e = 1$ means approval from the server for $e$ joining FL task $T$ and  $d_e = 0$ for rejection.
% % It is worth noting that only $K$ clients will be selected, thus $\sum_{e=1}^E d_e = K$.
% and provide corresponding prices $p_e$ for them, denoted as $\mathbb{P} = \{p_e\}_{e \in S}$, which is anticipated to be a critical price in a truthful auction mechanism. The following illustrates the selection and pricing algorithm.





\myparagraph{Top-K Client Selection and Pricing}
\label{subsec:selectandprice}
% \begin{algorithm}[t]
%     \caption{Top-K Selection and Pricing in \projecttitle}
%     \label{algorithm1}
%     \textbf{Input:} Bids $\mathbb{B} = \{b_e\}_{e \in \mathbb{E}}$ and Scores $\mathbb{U^T} = \{u_e^T\}_{e \in \mathbb{E}}$\\
%     \textbf{Output:} Decisions $\mathbb{D} = \{d_e\}_{e \in \mathbb{E}}$ and Prices $\mathbb{P} = \{p_e\}_{e \in \mathbb{E}}$\\
%     \textbf{Top-K winners selection}\\
%     $\mathbb{V}\leftarrow \mathbb{U^T}-\mathbb{B}$\\
%     $\mathbb{S} \leftarrow argsort(\mathbb{V},K)$  {\color{teal} \raggedright \footnotesize{\null\hfill Return the indices of top-K values}}\\ 
%     $I_{K+1} \leftarrow argmax(\mathbb{V},K+1)$ {\color{teal} \raggedright \footnotesize{\null\hfill Return the index of the $K+1$-th maximum value}}\\ 
%     $\mathbb{D}=\{d_e\}_{d_e=1,e\in \mathbb{S}; d_e=0,e\notin \mathbb{S}}$\\
%     \textbf{Price determination}\\
%     $\Delta=\{ \delta_e\}_{\delta_e=v_e-v_{I_K+1}}$\\
%     $\mathbb{X}=\{x_e\}_{x_e=b_e+\delta_e,v_e>0;x_e=u_e^T,v_e\leq 0}$\\
%     $\mathbb{P}\leftarrow \mathbb{D}\cdot \mathbb{X}$\\
% \Return{$\mathbb{D}$ and $\mathbb{P}$}
% \end{algorithm}
\lei{According to $\mathbb{B} = \{b_e\}_{e \in \mathbb{E}}$ and $\mathbb{V} = \{v_e\}_{e \in \mathbb{E}}$, the server determines $K$ the number of clients to be selected under budget $B$ and select the Top-K winners from $\mathbb{E}$. Moreover, the server determines the final price $p_e$ for the winners, denoted as $\mathbb{P} = \{p_e\}_{e \in S}$, which is anticipated to be a critical price in a truthful auction mechanism. The following illustrates the selection and pricing algorithm.}
% According to $\mathbb{V} = \{v_e\}_{e \in \mathbb{E}}$, the server $S$ selects top-K winners from $\mathbb{E}$, 
% and provides corresponding payment $p_e$ for them, denoted as $\mathbb{P} = \{p_e\}_{e \in S}$, which is anticipated to be a critical price in a truthful auction mechanism. The following illustrates the selection and pricing algorithm.


\emph{Algorithm Design:}
We propose a greedy top-K selection and payment algorithm, which is guaranteed to provide the critical value for each client $e$ and thus achieves the \textit{truthful} property of our auction mechanism~\cite{yang2012crowdsourcing}.
The detailed steps of the winner selection phase and \lei{price} determination phase are shown in Algorithm~\ref{algorithm1}. 
The algorithm gets the inputs of $\mathbb{B}$ and $\mathbb{U^T}$, which are the bids set and pricing set of all clients $\mathbb{E}$. 
% For the selection phase of Algorithm~\ref{algorithm1}, the server $\mathbb{S}$ selects the top-K clients with the largest utility values $v_e$ (line 5) and records the client's index with the largest $K+1$ value of utility, denoted as $I_{K+1}$ (line 6). 
% To determine the critical price of each selected client, we first calculate the difference between its utility value and the recorded $I_{K+1}$ client (line 23).
% Then we add the difference value to each client's bid to get its critical price $p_e$. 
% Finally, the server returns the output decisions $\mathbb{D}$ and critical prices $\mathbb{P}$ for all clients $\mathbb{E}$.
\lei{At the begin of Algorithm~\ref{algorithm1},the server $S$ sorts the clients with its $b_e/u_e^T$ (line 3). Then the server adds up the bids in turn until it exceeds the budget $B$ (line 7). After that, the server determines the participating clients and their utility values (line 10). 
To determine the critical price of winners, the server determines $(K+1)$-th utility value $v_{K+1}$ as the markup ratio for winners, i.e. $p_e = v_{K+1} \times u_e^T$, which critical price also is the payment that the server determined.
Finally, the server determines the winners $\mathbb{S}$ with its price $\mathbb{P}$ and publishes to clients.
}
% For the selection phase of Algorithm~\ref{algorithm1}, the server $S$ sorts the clients with its $b_e/u_e^T$ (line 3), and selects the top-K largest utility values $v_e$ (line 6). Then records selected clients $\mathbb{S}$ (line7).
% To determine the critical price of winner clients, we first calculate the difference between its utility value and the $(K+1)$-th value (line 11).
% Then we add the difference value to each client's bid to get its critical price $p_e$ (line 12), which also is the payment that the server determined. After that, we get the payment for winners $\mathbb{P}$. Finally, the server returns the selected clients $\mathbb{S}$ and payment $\mathbb{P}$ for them.

\begin{algorithm}[h]
    \caption{Top-K Selection and Pricing}
    \label{algorithm1}
    \textbf{Input:} Bids $\mathbb{B} = \{b_e\}_{e \in \mathbb{E}}$ and Prices $\mathbb{U^T} = \{u_e^T\}_{e \in \mathbb{E}}$\\
    \textbf{Output:} Selected clients $\mathbb{S}$ and Payment $\mathbb{P}$\\
    Sort $e\in \mathbb{E}$ $s.t.$ $b_1/u_1^T<...<b_e/u_e^T<...<b_E/u_E^T$\\
    $\mathbb{B}\leftarrow \{b_1,...,b_e,...b_E\}$; $\mathbb{U^T}\leftarrow \{u_1^T,...,u_e^T,...,u_E^T\}$\\
    $\mathbb{V}\leftarrow \{b_e/u_e^T\}_{e\in \mathbb{E}}$\\
    $sum \leftarrow 0$; $K \leftarrow 0$; $\mathbb{S}\leftarrow \emptyset$\\
    \textbf{K and Top-K winners determination:}\\
    \For{$b_e$ in $\mathbb{B}$ and $v_e$ in $\mathbb{V}$}{
        \If{$(sum \leftarrow sum+b_e) \leq B$}{
            $K\leftarrow K+1$;\\
            $\mathbb{S}\leftarrow \mathbb{S} \bigcup \{K\}$
        }
        % \Else{
        %     break
        % }
    }
    \textbf{Payment determination:}\\ 
    \For{$e$ in $\mathbb{S}$}{
        $p_e=u_e^T\times v_{K+1}$
    }
    $\mathbb{P} = \{p_e\}_{e\in \mathbb{S}}$\\
    % \For{$v_e$ in $\mathbb{V}_s$}{
    %     % \If{$v_e>0$}{
    %         $\delta_e \leftarrow v_{K+1} - v_e$\\
            
    %         $p_e\leftarrow b_e+\delta_e$, (If $\delta_e \geq 0)$; $p_e\leftarrow b_e$,(If $\delta_e < 0$)\\
    %     % }
    %     % \Else{
    %     %     $p_e\leftarrow u_e^T$\\
    %     % }
    % }
\Return{$\mathbb{S}$ and $\mathbb{P}$}
\end{algorithm}

\myparagraph{A Walk-through Example}
Let us consider an example involving a client pool of 5 clients with a budget of 14 shown in Figure~\ref{fig:auction_example}.  
\lei{After calculating the price and getting bids from all clients in $\mathbb{E}$, we obtain $\mathbb{B} = \{3,4,5,3,4\}$ and $\mathbb{U^T} = \{2, 3, 3,3,2\}$. 
Next, we calculate $b_e/u_e^T$ and sort them, the sorted utility values for all clients as $\mathbb{V} = \{v_1= 1, v_2= 1.3, v_3= 1.5, v_4= 1.7, v_5= 2\}$, and the corresponding $\mathbb{U^T}=\{u_1^T=3,u_2^T=3,u_3^T=2,u_4^T=3,u_5^T=2\}$, $\mathbb{B}=\{b_1=3,b_2=4,b_3=3,b_4=5,b_5=4\}$. 
Then add $b_1,b_2,b_3,...$ in sequence, when adding $b_4$, the sum of the bid is 15 which is greater than the budget $B=14$. Based on that we select clients whose combined bids do not exceed the budget as the winners and determine the $K$, i.e., $\mathbb{S}=\{1,2,3\},K=3$.
To determine the final price for each of the winning clients, we take the $K+1$-th utility value ($v_{K+1}=1.7$) as the markup ratio. Then multiply the price by the markup rate for the final price, i.e., $\mathbb{P}=\{5.1,5.1,3.4\}$. 
Finally, we obtain the selected clients $\mathbb{S}$ and the corresponding prices $\mathbb{P}$.
}
\begin{figure}[t]
\vspace{-3mm}
\centering
% \includegraphics[width=0.26\textwidth]{./figuresTex/auction_example.pd`f}
\includegraphics[width=0.45\textwidth]{./figuresTex/figs/auction_new.pdf}
\vspace{-3mm}
 %\caption{A Walk-through Illustration of Top-K Selection and Pricing in \projecttitle}
 \caption{A walk-through illustration of top-K selection and pricing in \projecttitle}
\label{fig:auction_example}
\vspace{-5mm}
\end{figure}

\myparagraph{Truthful Property of The Bidding Mechanism}
\label{sec:truthful}
Now we show that our bidding mechanism with Algorithm~\ref{algorithm1} is truthful.
\begin{lemma}~\cite{singer2010budget}
A bidding mechanism is truthful if and only if:
\begin{enumerate}
    \item The selection algorithm is monotone, i.e. If $e$ wins the bidding by $b_e$, it will also win by bidding $\hat{b}_e < b_e$;
    \item Each winner is paid at the critical value: $e$ would not win the bidding if $\hat{b}_e > p_e$.
\end{enumerate}
\end{lemma}
% \textbf{Theorem 1.} Algorithm~\ref{algorithm1} is truthful if and only if~\cite{singer2010budget}:
% \begin{enumerate}
%     \item The selection algorithm is monotone, i.e. If $e$ wins the auction by $b_e$, it will also win by bidding $\hat{b}_e < b_e$;
%     \item Each winner is paid at the critical value: $e$ would not win the auction if $\hat{b}_e > p_e$.
% \end{enumerate}
\begin{theorem}
    Algorithm~\ref{algorithm1} is truthful
\end{theorem}
\begin{proof}
    Firstly, we consider the requirement that the selection algorithm should be monotone. In Algorithm~\ref{algorithm1}, we greedily select the top-K clients according to their utility value $v_e$, which is calculated by $v_e = b_e/u_e^T$. If a client $e$ wins the bidding by $b_e$, it also will win by bidding as $\hat{b}_e < b_e $ since $\hat{v}_e < v_e$.

    We next show that each client $e$ is priced at the critical value $p_e$. Considering a winner client $e$ require a payment $\hat{b}_e > {p}_e$. Then the new utility value is $\hat{v}_e = \hat{b}_e/u_e^T$. Comparing $\hat{v}_e$ and $v_{I_{K+1}}$, we have $\hat{v}_e < v_{I_{K+1}}$ since 
    \begin{align*}
    \hat{v}_e - v_{I_{K+1}}
    &= u_e^T - \hat{b}_e - v_{I_{K+1}} \\
    &< u_e^T - p_e - v_{I_{K+1}} = u_e^T - (b_e + \delta_e) - v_{I_{K+1}}\\
    &= u_e^T - (b_e + v_e - v_{I_{k+1}}) - v_{I_{K+1}} = 0
    \end{align*}
    Therefore the rank of $e$ will fall behind client $I_{K+1}$, resulting that $e$ will lose the bidding and client $I_{K+1}$ will be selected instead. In another word, it will be replaced after $K$ if $e$ submits a bid with $\hat{b}_e > {p}_e$.
\end{proof}


% \begin{itemize}
%     \item \emph{After a FL training task starts, there are no new clients allowed to submit their bids. }
%     \item \emph{}
% \end{itemize}

==> challenge.tex <==
\subsection{Challenges and Observations}

On one hand, a client would not like to participate in an FL training task, unless it receives a satisfying reward to compensate for its shared data and usage of computing resources. On the other hand, the server would like to select the "best" group of clients that can maximize the global model's accuracy. The following discusses the challenges to achieving the above-mentioned goals. 

\myparagraph{The incentive mechanism for an FL task}
Giving a satisfactory reward is the key to incentive a client to participate in an FL task. 
To this end, auction~\cite{klemperer1999auction} offers a solution to allow the server to obtain the clients' expected payments. 
However, some clients may be selfish and will ask for a reward that much higher than their contributions. This dishonest behavior undermines the integrity of the auction process and can lead to the server failing to obtain the real market price for performing the FL task, causing an unfair outcome. 
Thus, the difficulties in designing the auction mechanism are 
\emph{ 
1) The proposed mechanism needs to ensure the truthful bid of each client, and the server, therefore, can obtain the real market price for an FL task. 
2) Based on this price and the clients' bid, the server determines the payment to maximize the high-quality clients' demand to incentive them to join the FL task. 
} 
To this end, our auction mechanism needs to have the following properties. 
\begin{itemize}
\item \myparagraph{Truthful} 
An auction is truthful in bidding price if and only if each client’s reward is maximized when it bids with its true cost

\item \myparagraph{Incentive} To encourage the clients to join an FL task,  the payment for each selected client must be higher than its bid and the total payment should not exceed the budget.
\end{itemize}





\begin{figure}[t]
\centering
    \subfloat[Data Quantity]{
    \includegraphics[height=.18\textwidth]{./figuresTex/figs/Amountandacc.pdf}
    \label{fig:Amountandacc}}
    \subfloat[Data Balance]{
    \includegraphics[height=.18\textwidth]{./figuresTex/figs/motivation_data.pdf}
    \label{fig:motivation_data}}
    %\subfloat[Free rider attack]{
    %\includegraphics[width=.28\textwidth,height=0.192\textwidth]{./figuresTex/figs/motivation_fake.pdf}
    %\label{fig:motivation_fake}}
    \caption{The Impact of Data Quantity and Distribution for Training an FL Training Task}
    \label{fig:dsads}
    \vspace{-4mm}
\end{figure}

\myparagraph{The high-quality clients for training an FL task}
\label{sec:finding}
Valuing the data of a client before actually performing the training task is non-trivial. 
To investigate the impact of two factors of data, i.e. quantity and distribution, we conduct the following experiments.
% Scoring the bid which consists the data statistics of a client is non-trivial for both providing better clients for the server and incentiving potential clients contributing to the FL task.
% However, evaluating the data is challenging since (i) The quantity of data could not fully represent the value of the data;
% (ii) The measurement of data quality (e.g.scarcity) is hard to measure \di{This sentence need to be rephrased};
% (iii) privacy concerns in the scoring procedure are also existed thus should be fairly addressed \di{Probably not needed here}.
% To motivate the design of scoring function in \projecttitle, we experimentally investigate the impact of two factors of data, i.e. quantity and balance.
% we analyze the results of final accuracy under different data sizes and levels of imbalance, which lead to two key considerations for the scoring function for \projecttitle (Section \ref{sec:data_evaluation}). 

\myparagraph{Experiment Setting} For all experiments, We trained a popular ResNet-56~\cite{he2016deep} model using CIFAR-10~\cite{krizhevsky2012imagenet} dataset. In particular, for FL training, we adopt FedAvg~\cite{mcmahan2017communication} as the aggregation algorithm with the following hyper-parameters setting, total rounds are 600; batch-size equals 128; learning rate is 0.003; the weight decay is set to 0.001.

% \textbf{Data quantity.}
To investigate the impact of data quantity, we examine the test accuracy of global models that are trained upon different volumes of data on each client. 
In practice, we obtain 100 global models trained with the data size equally varying from 100 to 10,000 on each client. 
We report the accuracy and its changes ($\Delta Accuracy$) for every 1,000 incremental data. 

\myparagraph{Finding-1: the accuracy of the global model is positively correlated to the size of data with a diminishing trend of marginal accuracy}
Figure~\ref{fig:Amountandacc} shows the curve of test accuracy against the volume of data and bars of $\Delta Accuracy$ for every 1,000 incremental data. 
From the results, we could observe that the test accuracy increases with the increase in the amount of training data. 
However, the accuracy gain for every 1,000 incremental data decreases rapidly, indicating that the marginal contribution of data to the test accuracy is limited when the data size is large.

% \textbf{Data Imbalance}
To evaluate the impact of data distribution, we compare the model accuracy under different distributions. 
(i) The data distribution is balanced for each client. Moreover, if we aggregate them all together on the server, the global distribution is also balanced, namely \textit{local balance and global balance}. 
(ii) The data distribution is imbalanced for each client. However, if the global distribution is balanced when combining them together, namely \textit{local imbalance and global balance}. 
(iii) Both the local data distribution and global data distribution are imbalanced, namely \textit{local imbalance and global imbalance}. 
In particular, we build an FL test bed with 20 clients with the aforementioned different levels of data imbalance and keep the number of total data among all clients the same (i.e. 32,000) to exclude the impact of the data size. We report the test accuracy of the FL training under the above setting to verify the impact of data imbalance.

\myparagraph{Finding-2: data imbalance can significantly deteriorate the accuracy of FL training. However, global balance can largely compensate for the degradation caused by the local imbalance}
Figure~\ref{fig:motivation_data} shows the results of FL training under three different levels of data imbalance. 
It is observable that the data imbalance significantly deteriorates the learning performance of FL training. For instance, when the FL model is trained with \textit{local imbalance and global imbalance} setting, the final accuracy  drops dramatically from 87\% to 74\% when compared with the FL model trained with balanced data. 
However, when the global data is balanced while the local data is still imbalanced (the green curve in Figure~\ref{fig:motivation_data}), the accuracy degradation for FL training is much milder; 
there is merely a 1\% accuracy loss lower than the ideal balance situation. 
In the practical scenario, the data imbalance is determined by the characteristics of end users, and hence cannot be controlled by the central server. Fortunately, the global distribution could be adjusted in the client selection process to mitigate the issue of local data imbalance.

==> evaluation.tex <==
% \begin{table}[h] 
% % \resizebox{0.3\textwidth}{!}{  
% \caption{Statistical information of datasets.}
% \centering
% \begin{tabular}{cccc}
% \toprule
%     \textbf{Application} &\textbf{Dataset} & \textbf{Number of clients} & \textbf{Classes} \\
%     \specialrule{0.05em}{2pt}{2pt} 
%   \multirow{2}{*}{CV}  & CIFAR10 & 20 and 100 & 10 \\
%      & CINIC10 & 20 & 10 \\

%     \specialrule{0.05em}{1.5pt}{1.5pt}   
%     HAR & DSADS & 20 &19 \\
%     \bottomrule
% \end{tabular}
% % }
% \label{dataset_list}
% \end{table}
% \begin{table}[t] 
% % \resizebox{0.3\textwidth}{!}{  
% \caption{Statistical Information of Datasets.}
% \centering
% \small
% \begin{tabular}{ccc}
% \toprule
%     \textbf{Application} &\textbf{Dataset}  & \textbf{Classes} \\
%     \specialrule{0.05em}{2pt}{2pt} 
%    \multirow{2}{*}{IC}  & CIFAR10  & 10 \\
%      & CINIC10  & 10 \\

%     \specialrule{0.05em}{1.5pt}{1.5pt}   
%     HAR & DSADS &19 \\
%     \bottomrule
% \end{tabular}
% % }
% \label{dataset_list}
% \end{table}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.35\textwidth]{./figuresTex/figs/distributionlist.pdf}
%     \caption{Distribution list of CIFAR10}
%     \label{fig:Distribution list}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.35\textwidth]{./figuresTex/figs/dis_example.pdf}
%     \caption{Allocating CIFAR10-D7 into Clients}
%     \label{fig:dis_example}
% \end{figure}


\begin{figure*}[t]
\centering
    \subfloat[Distribution List of CIFAR10]{
    \includegraphics[width=0.40\textwidth]{./figuresTex/figs/distributionlist.pdf}
    % \caption{Caption}
    \label{fig:Distribution list}
    }
    \subfloat[Allocating CIFAR10-D6 into Clients]{
     \includegraphics[width=0.393\textwidth]{./figuresTex/figs/dis_example.pdf}
    % \caption{Caption}
    \label{fig:dis_example}
    }
    \vspace{-1mm}
    \caption{The Generated Data Distributions of CIFAR10 and an Example of its Allocation}
    \label{fig:data_distribution}
    \vspace{-3mm}
\end{figure*}




\section{Evaluation}
\label{sec:evaluation}

\subsection{Experimental Setup}
\label{sec:expsetup}

\myparagraph{Applications, Datasets and Models}
To demonstrate \projecttitle's generalizability across different applications and models, we evaluate \projecttitle on two representative AI applications that can benefit significantly from FL.

\begin{itemize}[leftmargin=10pt]
    \item \textbf{Application\#1: Image Classification (IC)} Image classification has been applied to many real-world applications such as disease diagnosis, and city surveillance where FL can help to prevent sensitive data leakage. In this work, we use CIFAR10~\cite{krizhevsky2009learning} and CINIC10~\cite{darlow2018cinic} datasets for training and evaluation. Resnet56~\cite{he2016deep} is used as a base training model for both 10-class image classification tasks.   
    \item \textbf{Application\#2: Human Activity Recognition (HAR)} Human activity recognition based on data collected from wearable devices and smartphones is a revolutionary technology for personal health detection and is widely used in medical rehabilitation, safe driving, etc. In this work, we use the DEAP~\cite{koelstra2011deap} dataset which collects electroencephalogram (EEG) and
    peripheral physiological signals from 32 participants when watching long music videos. We generate training samples by filtering and transforming EEG data, and build a simple classification task for predicting likeness levels, ranging from 1-9. We build a light-weight customized three-layer CNN model with a softmax layer for a 9-class likeness prediction task.
\end{itemize}

% \vspace{-5mm}
\myparagraph{The Data Distribution of Clients} In real-world FL tasks, the data distribution of each client is not exactly the same and follows the non-i.i.d. distribution.  
% \cite{} indicates that data distribution of clients are Non-IID which follows dirichlet distribution.
We, therefore, perform the following two-step strategy that first generates $M$ datasets with different distributions and then distributes each dataset to $k$ clients.


\begin{itemize}[leftmargin=10pt]
    \item \textbf{Data distribution generation:} To comprehensively evaluate our algorithm, we generate $M$ datasets and each one has a different distribution.
    We first obtain $D$ from the original dataset that is evenly distributed across the target classes. For example, an original dataset <50,000, 10> includes 10 classes and each class has 5,000 samples, which is denoted as D1. Based on D1, we then sequentially delete an incremental number of samples for each class to create uneven distributions. Figure~\ref{fig:Distribution list} shows an example of data generation for CIFAR10, where \emph{Class} represents the class type and \emph{Distribution} indicates that we generate 6 data distributions. 
    
    \item \textbf{Allocating data to clients:} For each experiment, we allocate one generated dataset to $k$ clients.
    Following the settings in \cite{hsu2019measuring}, we simulate the non-i.i.d. data distribution for all clients by drawing allocations from a Dirichlet Distribution Dir($\alpha D_{n}$), where $\alpha$ is a concentration parameter controlling the identicalness of the clients and $D_{n}$ is the prior distribution generated in the first step. 
    We set $\alpha=0.5$ for all allocations and figure~\ref{fig:dis_example} shows an example that allocates D6 to 20 clients with CIFAR10. 
\end{itemize}

% \myparagraph{Data and Client Heterogeneity} To evaluate the efficacy of \projecttitle under different conditions, we follow a two-step strategy to generate various data distributions and distribute the data to the clients.
% \begin{itemize}[leftmargin=10pt]
%     \item \textbf{Data heterogeneity:} We first generate various number of data distributions, D = \{$D_{1}$ ... $D_{N}$\} from the original datasets. 
%         The original datasets contain  <50,000, 10>,  <90,000, 10> and <90,000, 9> samples that are evenly distributed across the target classes. 
%         Thus, D1 is a uniform distribution that contains 5000, 9000 and 10000 samples for each class in CIFAR10, CINIC10 and DEAP.
%         Based on D1, we then sequentially delete incremental number of samples for each class to create uneven distributions.  
%         Figure~\ref{fig:Distribution list} shows an example of data generation for CIFAR10, where \emph{Class} represents the class type and \emph{Distribution} indicates that we generate 6 data distributions. 
%         D6 is the skewest distribution, with only 500 samples for C9 and 5000 samples for C0, indicating an arithmetic progression between 500 and 5000 samples.
%         All generations follow the same strategy and we finally get 6, 7, and 6 distributions for three datasets respectively. \zy{may give a reason why we use 6, 7, 6}
%     \item \textbf{Client heterogeneity:} We further allocate the generated data distributions into different clients. 
%        Following the settings in \cite{hsu2019measuring}, we simulate the non-i.i.d. data distribution for all clients by drawing allocations from a Dirichlet Distribution Dir($\alpha D_{n}$), where $\alpha$ is a concentration parameter controlling the identicalness of the clients and $D_{n}$ is the prior distribution generated in the first step. 
%        We set $\alpha=0.5$ for all allocations and figure~\ref{fig:dis_example} shows an example allocation of CIFAR10, D6 over 20 clients. 
% \end{itemize}


\begin{figure*}[t]
\centering
    \subfloat[5 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cf20x5.pdf}
        \label{fig:cf20x5}}
    \subfloat[10 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cf20x10.pdf}
        \label{fig:cf20x10}}
    \subfloat[15 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cf20x15.pdf}
        \label{fig:cf20x15}}
    \vspace{-1mm}
    \caption{CIFAR10: $n$ Clients Selected from 20 Clients}
    \label{fig:cifar}
    \vspace{-4mm}
\end{figure*}

\begin{figure*}[t]
\centering
    \subfloat[5 clients selected]{
      \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cn20x5.pdf}
    \label{fig:cn20x5}}
    \subfloat[10 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cn20x10.pdf}
    \label{fig:cn20x10}}
    \subfloat[15 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cn20x15.pdf}
    \label{fig:cn20x15}}
    \vspace{-1mm}
    \caption{CINIC10: $n$ Clients Selected from 20 Clients}
    \label{fig:cinic}
    \vspace{-3mm}
\end{figure*}

\begin{figure*}[t]
\centering
    \subfloat[5 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/dsa20x5.pdf}
    \label{fig:dsa20x5}}
    \subfloat[10 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/dsa20x10.pdf}
    \label{fig:dsa20x10}}
    \subfloat[15 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/dsa20x15.pdf}
    \label{fig:dsa20x15}}
    \caption{DEAP: $n$ Clients Selected from 20 Clients}
    \label{fig:deap}
    \vspace{-4mm}
\end{figure*} 


\begin{figure*}[t]
\centering
    \subfloat[25 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cf100x25.pdf}
    \label{fig:cf100x25}}
    \subfloat[50 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cf100x50.pdf}
    \label{fig:cf100x50}}
    \subfloat[75 clients selected]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/cf100x75.pdf}
    \label{fig:cf100x75}}
    \caption{CIFAR10: $n$ Clients Selected from 100 Clients}
    \label{fig:cifar10x100}
    \vspace{-4mm}
\end{figure*}

% Table~\ref{dataset_list} lists the statistics of the datasets that are used to build the applications. 





\myparagraph{Baselines}
We compare \projecttitle with four baselines in the literature that can be applied to select the clients before the training phase.

\begin{itemize}[leftmargin=10pt]
    \item \emph{Diversity-driven Selection (DDS)}: \cite{li2021sample} proposed a client selection strategy that enforces high statistical homogeneity of on-device data samples and content diversity across different clients. A novel content embedding representation technique is developed to distinguish data content between different clients.  Thus, the selected clients tend to hold an even number of samples among all categories and are diverse in data content, such to increase the training performance.
    \item \emph{DICE}: \cite{saha2022data} aims to select potential clients who have large amounts of data and exhibit significant heterogeneity among their datasets compared to others. A data quality ratio is used to select high-quality clients to participate in FL training, calculated by dividing data volume by the data heterogeneity coefficient.
    \item \emph{Random Selection (RS)}: The central server randomly selects a fixed number of clients to conduct FL training.
    \item \emph{Quantity Based Selection (QBS)}: \cite{zeng2020fmore} proposed a client selection method that selects a fixed number of clients based on their data volumes in descending order.
\end{itemize}

In addition, most of the existing client selection algorithms in FL are applied during the training phase, which selects the clients based on the updated local models \cite{lai2021oort, nagalapatti2021game}, and is not suitable for pre-training pricing.  In section~\ref {sec:in-training}, we compare the performance of our \projecttitle with the SOTA in-training client selection method i.e., S-FedAvg~\cite{nagalapatti2021game}.

%move to the implementation

\myparagraph{Hardware and Parameters} Our experiments are conducted on a Linux Server with 40-core 4.0 GHz Intel Xeon CPU and 8 NVIDIA V100 GPUs. 
For the server side, we configure a docker container with 8 CPU cores and 1 GPU, and the clients equally share the rest of the computing resources.  
The implementation is based on Pytorch and FedML~\cite{he2020fedml}.

The batch size during training is 128, and 64 for experiments with 20 and 100 clients respectively.
For CINIC10, the initial learning rate is 0.001 and the weight decay factor is 0.0005.
For CIFAR10 and DEAP, the initial learning rate is 0.003, and weight decay is 0.001.
All client models are aggregated after each training round and we perform training for 600 rounds in total.


\myparagraph{Evaluation Metrics} We evaluate the performance of each method by the inference accuracy of the trained global models. 


% We evaluate our \projecttitle in terms of generality and efficiency. Thus, we apply our \projecttitle to various types of datasets under different conditions, while comparing with other baselines. 



% \begin{table}[t]
% \noindent

% \renewcommand\tabcolsep{5.5pt}
% \caption{Distribution list of CIFAR10}
% \resizebox{0.49\textwidth}{!}{  
% \label{Distribution list}

%     \begin{tabular}{c|cccccccccc}
    
%     \toprule
%     \diagbox[innerwidth=1.2cm]{Dis}{Class}&0&1&	2&	3&	4&	5&	6&	7&	8&	9\\
%     \specialrule{0.05em}{0.1pt}{3pt}
%     D1&	500&	1000&	1500&	2000&	2500&	3000&	3500&	4000&	4500&	5000\\
%     D2&	1400&	1800&	2200&	2600&	3000&	3400&	3800&	4200&	4600&	5000\\
%     D3&	2300&	2600&	2900&	3200&	3500&	3800&	4100&	4400&	4700&	5000\\
%     D4&	3200&	3400&	3600&	3800&	4000&	4200&	4400&	4600&	4800&	5000\\
%     D5&	4100&	4200&	4300&	4400&	4500&	4600&	4700&	4800&	4900&	5000\\
%     D6&	5000&	5000&	5000&	5000&	5000&	5000&	5000&	5000&	5000&	5000\\
%     D7&	5000&	4500&	4000&	3500&	3000&	2500&	2000&	1500&	1000&	500\\
%     D8&	5000&	4600&	4200&	3800&	3400&	3000&	2600&	2200&	1800&	1400\\
%     D9&	5000&	4700&	4400&	4100&	3800&	3500&	3200&	2900&	2600&	2300\\
%     D10&	5000&	4800&	4600&	4400&	4200&	4000&	3800&	3600&	3400&	3200\\
%     D11&	5000&	4900&	4800&	4700&	4600&	4500&	4400&	4300&	4200&	4100\\
%     \bottomrule
    
%     \end{tabular}
%     }
% \end{table}


% \begin{table}[t]
% \noindent
% \renewcommand\tabcolsep{5.5pt}
% \caption{Allocating CIFAR10-D1 into Clients}
% \resizebox{0.49\textwidth}{!}{  
% \label{D1}


%     \begin{tabular}{c|cccccccccc}
%     \toprule
%     \diagbox[innerwidth=1.2cm]{Client}{Class}&0&1&	2&	3&	4&	5&	6&	7&	8&	9\\
%     \specialrule{0.05em}{0.1pt}{3pt}
%     Client1&	32&	210& 22& 87& 719& 2& 224& 477& 0& 0\\
%     Client2&	10&35&9&159&1&145&48&1&27&89	\\
%     Client3&	12&17&123&49&14&47&40&4&97&564 \\
%     Client4&	7&1&61&9&170&125&1&416&397&952 \\
%     Client5&	10&92&133&1&1&405&198&57&24&135 \\
%     Client6&	3&210&4&10&7&24&124&593&784&0\\ 
%     Client7&	5&19&36&11&1&72&55&76&65&580\\
%     Client8&	1&132&17&5&13&82&445&92&182&76\\
%     Client9&	11&65&24&25&103&161&427&110&259&1\\
%     Client10&	53&51&358&78&192&18&44&96&222&650\\
%     Client11&	23&1&17&1&121&70&473&65&180&267\\
%     Client12&	63&11&45&38&64&7&3&399&26&265\\
%     Client13&	20&11&224&190&15&22&129&103&13&202\\
%     Client14&	26&2&51&215&18&229&342&103&194&0\\
%     Client15&	2&4&201&110&74&167&63&76&2067&0\\
%     Client16&	33&19&4&99&606&138&6&52&853&0\\
%     Client17&	7&61&77&78&81&25&18&203&2&172\\
%     Client18&	45&74&20&512&13&110&884&0&0&0\\
%     Client19&	100&1&26&532&7&171&580&0&0&0\\
%     Client20&	37&3&53&378&288&609&380&0&0&0\\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \vspace{-2mm}
\subsection{Client Selection Evaluation}\label{sec:CSE}

In this section, we evaluate \projecttitle's performance in selecting high-quality clients by comparing the proposed algorithm with four baselines. 
Figure~\ref{fig:cifar}, \ref{fig:cinic}, and \ref{fig:deap} show the validation accuracy of \projecttitle for three datasets when selecting various numbers of clients from 20 clients.  
We also investigate the impact of the number of clients by increasing it from 20 to 100 and the experimental results are reported in Figure~\ref{fig:cifar10x100}.


\myparagraph{The Effectiveness of \projecttitle for Different Tasks} As shown in Figure~\ref{fig:cifar}, \ref{fig:cinic} and \ref{fig:deap}, \projecttitle outperforms other baselines (RS, QBS, DICE, DDS) on most cases, especially when the original data distributions is unbalanced (e.g., D4, D5, D6).
\projecttitle achieves 40.78 $\%$,  44.78 $\%$,  17.52 $\%$ and  47.05 $\%$ higher accuracy on CIFAR10, compared to other four baselines.
In the more complex dataset (CINIC10), we notice in Figure~\ref{fig:cinic} that \projecttitle reaches 28.10 $\%$,  31.74 $\%$,  5.44 $\%$ and  7.27 $\%$ higher accuracy. 
Comparing results in Figure~\ref{fig:cf20x5}, \ref{fig:cf20x10} and \ref{fig:cf20x15} for CIFAR10, when we select 10 clients out of 20, 
the performance gain of \projecttitle is more significant than selecting 5 and 15 clients (3.45 $\%$, 11.25 $\%$ and 6.53 $\%$) respectively.
A similar phenomenon is observed for CINIC10 dataset in Figure~\ref{fig:cn20x5}, \ref{fig:cn20x10} and \ref{fig:cn20x15}, where \projecttitle achieves an average of 0.96 $\%$, 1.71 $\%$ and 2.69 $\%$ higher accuracy than that of baselines when selecting 5, 10 and 15 clients.
Moreover, in some cases (e.g., Figure~\ref{fig:cn20x5}(a) D1, D2 and Figure~\ref{fig:cn20x10}(b) D1) that the data is more balance our algorithm does not show its advantage comparing to DICE and DDS. Due to the fact that when the number of selected clients is small and the global data distribution is balanced, it is not  hard for selecting high-quality clients, other baseline algorithms (e.g., DICE) can also achieve this goal. Therefore, the performance of \projecttitle will increase with the increase of the number of selected clients and the degree of imbalance in data distribution.  We discussed details in Section~\ref{sec:data distribution}.
% When less clients are selected for the training, the performance gap between \projecttitle and other baselines is more significant.
% This indicates that the clients with the highest quality data can be prioritized by \projecttitle.
% When less training data is available, selecting high-quality data is even more important.


% the increase of training data directly affects the selection of \projecttitle in the amount of data, and the benefit of \projecttitle choosing rare data will reduce.

% \zy{the more complex tasks require more training data to achieve certain accuracy.} (\zy{need more discussions})

Regarding DEAP dataset, Figure~\ref{fig:deap} shows that \projecttitle achieves 25.67 $\%$,  16.41 $\%$,  8.63 $\%$ and  29.21 $\%$  higher accuracy than other baselines. 
% From the results, \projecttitle is more effective on computer vision applications than HAR applications. 
% This is mainly due to the fact that the HAR benchmark application is simpler than that of IC, where all client selection methods can achieve quite high accuracy.
When selecting 5, 10, and 15 clients from 20, all three cases achieve an average accuracy of 68.04 $\%$, 75.57 $\%$, and 78.40 $\%$ respectively.
\projecttitle is more effective when the data is imbalanced.
For example in Figure~\ref{fig:dsa20x5}, our \projecttitle reaches 68.04 $\%$  and 10.71 $\%$, 4.79 $\%$, 4.98 $\%$, 14.12 $\%$ higher accuracy than that of baselines.
This is because D6 in DEAP dataset has a very imbalanced distribution across all 20 clients.




% due to the low data complexity of HAR, the performance of \projecttitle on DSADS is as not obvious as on CV. But \projecttitle also achieves 9.54 $\%$ and 4.36 $\%$ higher accuracy. This further illustrates the effectiveness of \projecttitle on classification tasks.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{./figuresTex/figs/distribution.pdf}
%     \caption{Distribution example}
%     \label{fig:distribution}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{./figuresTex/figs/dis.pdf}
%     \caption{Cifar10}
%     \label{fig:dis}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{./figuresTex/figs/dis_cinic10.pdf}
%     \caption{Cinic10}
%     \label{fig:dis_cinic10}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{./figuresTex/figs/dis_dsads.pdf}
%     \caption{DSADS}
%     \label{fig:dis_dsads}
% \end{figure}


\myparagraph{The Performance of \projecttitle on a Large Number of Clients} To investigate the robustness of \projecttitle in the case of large number of clients, we report the results by conducting the experiments that select 25, 50 and 75 clients from a client pool of 100 clients. 
Note that the overall data volume and distribution is the same as in Figure~\ref{fig:cifar}, while the number of clients increases in this experiment. 


Figure~\ref{fig:cifar10x100} demonstrates that \projecttitle outperforms other baselines, and achieves 14.66 $\%$, 22.06 $\%$, 5.19 $\%$ and 11.08 $\%$ accuracy improvement. 
However, comparing Figure~\ref{fig:cifar10x100} and \ref{fig:cifar}, when the client pool is enlarged and more clients are selected, the accuracy improvement of \projecttitle drops by 1-5 $\%$. This is because of selecting more clients increases the probability of baseline methods in selecting high-quality clients.
% This is mainly because when the same amount of data is allocated to more clients, each client gets less data, and the difference between the high-quality and low-quality clients is less significant.
% Also, selecting more clients increases the probability of baseline methods in selecting high-quality clients.

% Understandably, the model accuracy does not increase with the number of clients, where the average accuracy of 25 clients (see figure~\ref{fig:cf20x15}) and 75 clients (see figure~\ref{fig:cf100x75}) are xxx and xxx respectively.
% Moreover, \projecttitle outperforms other baselines. 

% Obviously, with large number of clients, the models' accuracy obtained from all evaluated methods have some improvements, and \projecttitle outperforms other baselines. 



% \myparagraph{Summary} The above experiments show the effectiveness of \projecttitle across various datasets, distributions and number of clients. Notably, the experimental results further validate the assumptions that 
% we made in \S \ref{sec:motivation}:  \emph{global data balance is beneficial to the improvement of model accuracy.}
% \bin{BIN: THIS conclusion is too strong to put here, data balance is not very distinct from figure 6,7,8,9}
% \zy{use the above experimental results to prove the assumptions of the paper.

\subsection{Convergence Speed.}\label{sec:CS}
 
We compare the convergence speed of \projecttitle with all the baselines. 
Figure~\ref{fig:my_convergence} shows that \projecttitle (red curve) converges much faster than baselines and has smaller training loss, consistently outperforming other approaches. For example, \projecttitle achieves 0.6 accuracy after only around 95 rounds, but DICE, DDS, QBS, and RS require 170, 380, 350, and 270 rounds, respectively, achieving a speedup of  1.31 $\times$, 2.92 $\times$, 2.69 $\times$, and 2.08 $\times$.

% \vspace{-5mm}
\begin{figure}[t]
\centering
    \subfloat[Accuracy Convergence]{
    \includegraphics[width=0.23\textwidth]{./figuresTex/figs/Accuracy.pdf}
    % \caption{Caption}
    \label{fig:my_acc}
    }
    \subfloat[Loss Convergence]{
     \includegraphics[width=0.23\textwidth]{./figuresTex/figs/Loss.pdf}
    % \caption{Caption}
    \label{fig:my_loss}
    }
    \vspace{-2mm}
    \caption{Convergence}
    \label{fig:my_convergence}
    \vspace{-5mm}
\end{figure}


\begin{figure}[t]
\centering
    \subfloat[Influence of Rarity]{
    \includegraphics[width=0.23\textwidth]{./figuresTex/figs/rarity.pdf}
    % \caption{Caption}
    \label{fig:test_theta}
    }
    \subfloat[Data Quantity Functions]{
     \includegraphics[width=0.23\textwidth]{./figuresTex/figs/function_exp.pdf}
    % \caption{Caption}
    \label{fig:test_phi}
    }
    \vspace{-2mm}
    \caption{Data Evaluation Function Tuning}
    \label{fig:data_evaluation_func}
    \vspace{-6mm}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{./figuresTex/figs/Accuracy.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{./figuresTex/figs/Loss.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure*}[t]
% \centering
%     \subfigure[xxxxxx]{
%     \includegraphics[width=0.45\textwidth]{./figuresTex/figs/rarity.pdf}
%     % \caption{Caption}
%     \label{fig:my_lack}
%     }
%     \subfigure[xxxxxxx]{
%     \includegraphics[width=0.45\textwidth]{./figuresTex/figs/function_exp.pdf}
%     % \caption{Caption}
%     \label{fig:my_func}
%     }
%     \caption{caption}
%     \label{fig:my_micro}
% \end{figure*}

\subsection{Effective Analysis of Evaluation Function.}\label{sec:sen_analysis}

We use specific dataset CIFAR10 to study the effectiveness of the evaluation function $\mathcal{U}_{e}$ as shown in Equation~\ref{eq:data_evaluation}. 11 distributions are configured from the dataset for evaluation.   

\myparagraph{The Impact of Data Rarity Coefficient $\theta_{c}$} To evaluate the effective of $\theta_{c}$, we conduct two types of experiments (i.e., with $\theta_{c}$ and without $\theta_{c}$). 
Figure~\ref{fig:test_theta} shows that the experiments with $\theta_{c}$ averagely reach 3.76 $\%$ higher accuracy than the experiments without $\theta_{c}$.
Furthermore, in the unbalanced distribution of D4 to D6 (see Figure~\ref{fig:Distribution list}), the improvement of $\theta_{c}$ is obvious, obtaining 7.89 $\%$ , 7.04 $\%$ and 8.92 $\%$ better accuracy than results without $\theta_{c}$. 
When the distribution is balanced, the values of $\theta_{c}$ for each class are nearly equal, adding $\theta_{c}$ may not bring a significant performance improvement as the experiments of D1 to D3 shown in Figure~\ref{fig:test_theta}. 
% and the accuracy of the two methods is close in the experiments of D10 and D11.
As a result, the effectiveness of $\theta_{c}$ reveals the importance of valuing rare data during client selection.

% This result reflects the meaning of the existence of $\theta_{c}$. 
% For a balanced dataset, all classes of data will be considered consistent. But in real environments, datasets are often unbalanced. Therefore, when conducting data evaluation, it is necessary for us to improve the score of data that is relatively scarce in the global data. 
% Conversely, those with normal data will also have lower scores. This will increase the probability of those clients with rare data being selected to some extent. And it can also avoid that all client data we selected are all normal data. In conclusion, $\theta_{c}$ can balance the scores of rare data and common data, so that the selected data set is as balanced as possible.


\myparagraph{Which is the ``Best'' Data Quantity Coefficient $\phi(n_{e}^{c})$} 
% \bin{BIN: We need to discuss this paragraph}
% \zy{we need to add why we compare with these functions. Also explain why our method is not perform well in D2 and D10}
$\phi(n_{e}^{c})$ measures the data quantity of each class over different clients, while reducing the rewards of clients which have large volumes of data. As we discuss in Section~\ref{sec:data_evaluation}, the function of $\phi(n_{e}^{c})$ needs to have feature that decreases as the number of data increases. Thus, we experimentally compares $f_{0}(x)=-\ln(x)$ with other functions, including linear function $f_{1}(x)=-x+1$ and quadratic function $f_{2}(x)=-x^2+1$ and $f_{3}(x)=(x-1)^2$. Also, these three comparison functions have  zero, negative and positive second derivatives that indicate the speed of the contribution decrease. Figure~\ref{fig:test_phi} shows that the functions with a positive second derivative outperform the other two functions. $f_{0}(x)=-\ln(x)$ achieves the highest accuracy 75.57 $\%$ that is 2.12 $\%$  higher than that of other functions.






% And their average accuracy are 70.59 $\%$, 70.92 $\%$ and 71.81 $\%$. We found that the function with a positive second derivative outperformed the other two functions. And $-\ln(x)$ is excellent for functions with positive second derivatives. Therefore the accuracy of using $-\ln(x)$ averagely is as high as 74.19 $\%$, achieves 3.1 $\%$ higher than that of other functions.}
% % 给个前提



% \begin{equation}
% \mathcal{U}_{e} = \sum_{c=0}^{C} \theta_{c} \cdot \phi(n_{e}^{c})
% \label{eq:data_evaluation}
% \end{equation}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.30\textwidth]{./figuresTex/figs/rarity.pdf}
%     \caption{Influence of rarity}
%     \label{fig:test_theta}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.30\textwidth]{./figuresTex/figs/function_exp.pdf}
%     \caption{Data quantity functions}
%     \label{fig:test_phi}
% \end{figure}
\begin{table}[t]
    \noindent
    \renewcommand{\arraystretch}{1.4}
    % \tabcolsep{5.5pt}
    % \caption{Clients Selected by \projecttitle}
    \caption{Selection Results of  \projecttitle and DICE CIFAR10-D6}
    \vspace{-3mm}
    \resizebox{0.48\textwidth}{!}{  
    \label{tabel5}
        \begin{tabular}{c|c|cccccccccc|c}
        \toprule
        \multicolumn{2}{c|}{ \diagbox[innerwidth=2.7cm]{Client}{Class}}&C0&C1&	C2&	C3&	C4&	C5&	C6&	C7&	C8&	C9&Distribution\\
        \specialrule{0.05em}{0.1pt}{3pt}
        \multirow{6}{*}{ Common}&Client 2&	9&203&19&224&224&318&362&40&0&0&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc1.pdf}\end{minipage}\\
        &Client 3&	5&120&112&311&472&58&0&319&360&0&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc2.pdf}\end{minipage}\\
        &Client 7&	6&125&66&14&207&75&6&97&121&36&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc6.pdf}\end{minipage}\\
        &Client 16&	151&378&29&4&85&44&125&12&69&174&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc15.pdf}\end{minipage}\\
        &Client 17&	30&42&171&201&11&1&322&111&53&70&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc16.pdf}\end{minipage}\\
        &Client 19&	33&212&23&99&29&64&141&109&157&25&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc18.pdf}\end{minipage}\\
        \specialrule{0.05em}{3pt}{3pt}
        \multirow{5}{*}{IPP}&Client 4&	220&11&2&46&659&0&55&16&169&143&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc3.pdf}\end{minipage}\\
         &Client 8&	401&11&56&6&724&66&36&5&25&6&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc7.pdf}\end{minipage}\\
         &Client 10&	1&244&13&93&4&83&52&191&1&25&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc9.pdf}\end{minipage}\\
         &Client 12&	287&9&42&65&13&5&114&600&45&21&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPAc11.pdf}\end{minipage}\\
         \cmidrule{2-13}
         &Sum& 1143&1355&533&1063&2428&714&1413&1500&1000&500&\begin{minipage}{0.1\textwidth}\includegraphics[width=20mm,height=5mm]{./figuresTex/figs/IPA.pdf}\end{minipage}\\
        \specialrule{0.05em}{3pt}{3pt}
        \multirow{5}{*}{DICE}&Client 1&	530&38&59&349&33&346&209&0&0&0&\begin{minipage}{0.1\textwidth}
        \includegraphics[width=20mm, height=5mm]{./figuresTex/figs/c1.pdf}\end{minipage}\\
         &Client 5&	281&174&211&4&247&570&0&0&0&0&\begin{minipage}{0.1\textwidth}
        \includegraphics[width=20mm, height=5mm]{./figuresTex/figs/c4.pdf}\end{minipage}\\
         &Client 13&	257&159&37&13&125&628&180&0&0&0&\begin{minipage}{0.1\textwidth}
        \includegraphics[width=20mm, height=5mm]{./figuresTex/figs/c6.pdf}\end{minipage}\\
         &Client 18&	2&605&43&133&166&271&398&0&0&0&\begin{minipage}{0.1\textwidth}
        \includegraphics[width=20mm, height=5mm]{./figuresTex/figs/c9.pdf}\end{minipage}\\
        \cmidrule{2-13}
         &Sum& 1304&2056&770&1342&1599&2345&1743&688&760&305&\begin{minipage}{0.1\textwidth}
        \includegraphics[width=20mm, height=5mm]{./figuresTex/figs/c.pdf}\end{minipage}\\
        \specialrule{0.05em}{3pt}{3pt}
        \multicolumn{1}{c|}{ IPP}&\multicolumn{2}{c|}{\multirow{2}{*}{Data Number} }& \multicolumn{2}{c|}{ 11449 } &\multicolumn{2}{c|}{ \multirow{2}{*}{Variance}}&\multicolumn{2}{c}{ 313880.1}&\multicolumn{2}{|c|}{ \multirow{2}{*}{Accuracy}}&\multicolumn{2}{c}{77.28 $\%$ }\\
        \cmidrule{1-1}\cmidrule{4-5}\cmidrule{8-9}\cmidrule{12-13}
        \multicolumn{1}{c|}{ DICE}&\multicolumn{2}{c|}{}& \multicolumn{2}{c|}{ 12912 } &\multicolumn{2}{c|}{}&\multicolumn{2}{c}{ 431920.6}&\multicolumn{2}{|c|}{}&\multicolumn{2}{c}{59.76 $\%$ }\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:selectedclients}
    \vspace{-6mm}
    \end{table}




\begin{figure*}[t]
\centering
    \subfloat[CIFAR10]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/sharpley_cifar10.pdf}
    \label{fig:sharpley_cifar10}}
    \subfloat[CINIC10]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/sharpley_cinic10.pdf}
    \label{fig:sharpley_cinic10}}
    \subfloat[DEAP]{
    \includegraphics[width=.3\textwidth,height=0.225\textwidth]{./figuresTex/figs/sharpley_deap.pdf}
    \label{fig:sharpley_deap}}
    \caption{Comparison of Performance between IPP and S-FedAvg across Three Datasets}
    \label{fig:sharpley_value}
    \vspace{-4mm}
\end{figure*}



\begin{table*}[t]
    \noindent
    \renewcommand{\arraystretch}{1.5}
    \caption{Comparison of Functional Indicators between IPP with other Frameworks}
    \vspace{-3mm}
    \resizebox{0.98\textwidth}{!}{
        \begin{tabular}{ccccccccc}
        \toprule
        \textbf{Functional indicators}&  \textbf{Description}&  \textbf{IPP}&  \textbf{Fmore}\cite{zeng2020fmore} & \textbf{AFL}~\cite{zhou2021truthful} &  \textbf{AUCTION}~\cite{deng2021auction} & \textbf{DICE}\cite{saha2022data} & \textbf{DDS} \cite{li2021sample} \\
        \cmidrule{1-8}
        Pre-Training Auction and Incentive
        & Conducting FL task auctions before training to incentive client participation in FL training
        & \ding{52} &\ding{52} &\ding{52} &\ding{54} &\ding{54}& \ding{54} \\
        \cmidrule{1-8}
        Data Pricing and Client Selection
        & Evaluating client data and providing appropriate pricing and selection
        & \ding{52}&\ding{52} &\ding{52} &\ding{54} &\ding{54} &\ding{54} \\
        \cmidrule{1-8}
        Privacy-aware Client Evaluation
        & Considering client privacy protection in data evaluation
        & \ding{52}& \ding{52}&\ding{52} &\ding{52} &\ding{52} &\ding{52}\\
        \cmidrule{1-8}
        Client Stability and Loyalty
        & Providing advance pricing in large AI or edge task scenarios to increase client stability and loyalty
        & \ding{52}&\ding{54} &\ding{54} &\ding{54}  &\ding{54}&\ding{54}\\
        \cmidrule{1-8}
        Task Budget Control
        & Performing pricing before training, calculating expenses and revenue in advance, stabilizing server budget
        & \ding{52}&\ding{52} & \ding{52}& \ding{52}&\ding{54}&\ding{54}\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:comparsion of function}
    \vspace{-3mm}
\end{table*}



\subsection{The Data Distribution of Selected Clients}
\label{sec:data distribution}
In this section, we further analyze the effectiveness of client selection strategies by comparing the data distributions of the selected clients.
We compare the selection results of \projecttitle to the best-performed baseline DICE, when selecting 10 clients from a client pool of 20 clients on CIFAR10-D6.
Note that D6 is an extreme case with very imbalanced global data distributions (see Figure~\ref{fig:Distribution list}). 

As shown in Table~\ref{tab:selectedclients}, the two strategies select 6 same clients from the clients pool (i.e., 1, 2, 6, 15, 16, 18). 
Comparing the other 4 clients selected by two strategies, the choices of IPP contain all scarce classes: client 3, 7, 9 and 11 contain data samples for all classes, while clients selected by DICE (i.e., 0, 4, 12 and 17) omit these scarce classes (i.e., 7, 8 and 9).
From the result that \projecttitle outperforms DICE in validation accuracy, we make the following explanations.
In DICE, the data quality coefficient considers data quantity and the variance of local data within one client, which is inferior to our data quality formulation in Equation~\ref{eq:data_evaluation} in two folds:
1) When considering the importance of data quantity, DICE simply sums up the data volume on each client, while we give different values to individual data samples in each class, which better reveals the value of scarce data samples.
2) Our data rarity coefficient considers global non-iid data distribution, an extra coefficient that pays even more value to data samples in rarer classes.
Our selection strategy is closely aligned with our findings in Section~\ref{sec:finding}, thus leading to better accuracy.

Another finding we observe from Table~\ref{tab:selectedclients} is that, compared to DICE, \projecttitle selects clients with less data quantity and smaller variance across different classes. 
During the selection process, DICE only considers local data variance, while \projecttitle values global balanced distribution and tends to choose clients with scarce data samples.
Via such a strategy, we select more valuable samples with less price, saving computation and communication costs during the training process. 
\projecttitle is able to select clients to meet \emph{Goal2} discussed in Section~\ref{sec:data_evaluation}.


% \bin{
\subsection{Contrasting Pre-training and In-training Client Selection}\label{sec:in-training}
Although in-training client selection methods are not suitable for pre-training incentives, these methods can better measure the contributions of each participating client. In this section, 
% We have motivated the importance and validated the effectiveness of \projecttitle in selecting high-quality clients pre-training. 
% In this subsection, we show that \projecttitle can achieve comparable results to in-training client selection approaches while saving much training time.
we compare \projecttitle to S-FedAvg~\cite{nagalapatti2021game}, a method based on Shapley-value~\cite{shapley1971cores}, which is capable of selecting the best groups of clients from the client pool during training.
S-FedAvg samples a few clients in each training round for realizing FL training in practice. 
We then perform experiments of selecting 5 clients from 20 for all three datasets, and report the accuracy and training time in Figure~\ref{fig:sharpley_value}.
For a fair comparison, S-FedAvg also samples 5 clients during each training round.

Overall, \projecttitle achieves an average of 66.12\%, 61.75\%, and 68.04\% accuracy as compared to 66.67\%, 58.89\%, and 64.17\% accuracy by S-FedAvg, indicating that \projecttitle can achieve comparable or even better performance than in-training client selection approach.
Looking into the different data distributions, \projecttitle achieves better performance on [D3, D5, D6], [D1, D5, D6, D7], [D2, D3, D4, D6] respectively, more than half of the experiments.
In other cases where \projecttitle shows inferior performance, the final accuracy difference is mostly less than 5\% as well.

However, in terms of the training time, \projecttitle is much faster than S-FedAvg.
It takes S-FedAvg 603min, 223min, and 1354min to complete the 600 rounds of training, a 5X, 11X, and 2.5X more time than \projecttitle in CIFAR10, DEAP, and CINIC10 datasets respectively.
Despite that S-FedAvg already adapts the vanilla shapely-value-based client selection approach in sampling a small subset of clients, it is still computationally expensive, which requires comparing a client's contributions to the rest of the clients' contributions.



% validates the benefits of our approach in ensuring high-quality training with much less computation overhead. 

% }

==> introduction.tex <==
\section{Introduction}\label{sec:introduction}
Training deep learning models requires a significant amount of data as input to achieve human-level performance~\cite{krizhevsky2017imagenet,silver2016mastering,devlin2018bert}. However, in certain fields, data tends to be sensitive, e.g. banking and medical data, which requires careful handling of such data\cite{van2014systematic}. In addition, traditional centralized learning requires the collection of data from participating clients (e.g. hospitals and banks), which is difficult to achieve due to concerns related to user's privacy~\cite{shokri2015privacy}, company interests~\cite{van2014systematic} and legal regulations~\cite{voigt2017eu}. Federated learning (FL), on the other hand, emerges as a privacy-preserving method, which provides a promising way to address these challenges. FL enables the training of models while keeping the data local to the individual institutions or entities. Instead of sharing raw data, FL focuses on exchanging model updates, which allows multiple clients to collaboratively train a model without directly accessing each other's local data~\cite{mcmahan2017communication}.
Research and industrial efforts have largely focused on developing new training algorithms or systems to improve the performance and scalability of performing FL \cite{bonawitz2019towards,kairouz2021advances}. However, limited research so far has studied the integration between data providers (clients) and FL task publishers (servers) in a data marketplace.

Section \ref{subsec:pipeline} illustrates the life-cycle of cross-silo FL training in a data marketplace, where a server gathers a number of clients from a pool of available participants to train a satisfactory model. Thus, apart from designing efficient FL training algorithms or systems, another key challenge is selecting high-quality clients which can also impact the performance of training \cite{song2019profit,zeng2021comprehensive,zhan2021survey}. 

To help the task publisher select a number of high-quality clients, as a data marketplace, it needs to accomplish the following two points: 1) incentivizing the clients to participate; 2) profiling the quality (or value ) of clients for participating in a FL training task. A client is willing to take part in or contribute its data for a FL task, if or only if it receives a reasonable reward. Existing data sharing (or client selection) frameworks \cite{liu2020fedcoin,wang2019measure,song2019profit,zeng2021comprehensive,zhan2021survey} for FL consider providing rewards for participated clients based on their contributions and the participated clients are unaware of their own benefits before deciding to join the task.
This can be overcome by determining the payment of each participating client based on their profiling. However, profiling a client for a FL task is a challenge.  It is because the quality of a client is not only dependent on each client itself having sufficient data but also on the data distribution of all selected clients~\cite{li2022federated}. 


% \subsection{Motivation}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{./figuresTex/figs/big system.pdf}
%     \caption{The Pipeline of Federated Learning Task}
%     \label{fig:pipeline}
%     \vspace{-4mm}
% \end{figure}


% \myparagraph{The Pipeline of FL Task} FL task typically consists of four phases as shown in Figure~\ref{fig:pipeline}~\cite{deng2021auction}: 
% \circled{1} \textit{Task Publication}: The central server announces to all registered clients with metadata of the anticipate FL task, including essential information regarding the topic of the task (e.g. human activities classification), the type of data recruited (e.g. wearable sensor data) and the eligibility of participants (e.g., hardware and software requirements)~\cite{hu2020trading,bonawitz2019towards}. 
% \circled{2} \textit{Client Selection}: It is infeasible to include all clients during the training process since only a small subset of clients might meet the eligibility~\cite{bonawitz2019towards}. 
% Additionally, the limited budget of the central server places a demand on allocating valuable payments to high-quality clients~\cite{yu2020sustainable}. 
% Therefore, a client selection process is necessary for the FL pipeline. 
% In detail, all active clients decide whether to join the FL task according to the announced information from the central server. 
% The clients interested in participating in the task are required to upload statistics (e.g. quantity and distribution of categories) of their own data and system specifications of the devices (e.g. computation and communication capacities) for client selection in the server~\cite{nishio2019client}. 
% Training details will be sent to the eligible participants of the subsequent FL training. 
% \circled{3} \textit{Training}: All participants and the central server collaboratively train a global model iteratively using various FL aggregation algorithms (e.g. FedAvg~\cite{mcmahan2017communication}). 
% \circled{4} \textit{Reporting and Validation}: After each training round, including the end of the entire FL training process, participants report their updates (i.e. the updated weights of the model) and summaries of training (e.g. time consumption) to the central server. The central server conducts client validation and generates training logs for future reference. 

% \myparagraph{The Importance of Pre-training Incentives} 
% \di{
% In practice, an incentive mechanism is essential to motivate clients to participate in the FL task~\cite{zhan2021survey,zeng2021comprehensive,kairouz2021advances}. FL requires significant resource consumption, including computation power and bandwidth, which can be a undeniably cost for clients. 
% Thus, voluntary collaboration in FL is normally impractical~\cite{LUO2019601}. 

% The existing works on the FL incentive mechanism mainly focus on valuing contributions~\cite{liu2020fedcoin,wang2019measure,song2019profit,zeng2021comprehensive,zhan2021survey} of each individual client during or after the training phase, which may lead to the negative outcomes:
% 1) The contribution of users can only be evaluated after their participation in the FL training, lacking early estimation.
% 2) More importantly, clients may be hesitant to participate in the training process if they do not see any tangible rewards for their efforts.}

% Pre-training incentives in client selection are crucial in FL for several reasons:
% (1) By offering predictable rewards, incentives can strongly motivate clients to participate in the subsequent FL training, ensuring a higher participation rate.
% (2) Incentives can encourage clients to contribute high-quality and diversified data before training, ultimately leading to better training performance.
% (3) It increases the client's loyalty to continue to participate in the FL task until the end, which can speed up the convergence of training \cite{lai2021oort}, compared to the case that the participants are in dynamic changes. 

% \input{challenge}


% The challenges of developing an incentivized pre-training pricing framework for selecting clients to conduct an FL training task are summarized as follows.

%  \myparagraph{C1} \textit{Incentivizing clients to reach their optimal bidding price presents a significant challenge:}
%     Auction is a suitable mechanism to allow the clients and server to reach a price consensus for conducting an FL training task. There are two main obstacles to this process: first, clients tend to unrealistically pursue maximum returns if there is no limit on their bid; second, even if a client is rational, it is often impractical for them to accurately assess their maximum payment. To address this challenge, a truthful auction mechanism should be implemented, where the server provides well-designed rules for all rational clients to follow. This would enable them to automatically achieve the maximum reward they deserve based on the value they provided. However, designing an incentivization mechanism that achieves this goal is challenging.

%     \myparagraph{C2} \textit{Valuing clients in advance of FL training is difficult}: The high-quality clients are determined by both data quantity and distribution of the clients. Therefore, this is hard to design a valuing function that takes the statistic of the clients' data as input to compute the contribution of clients for an FL task before conducting the training process. Also, this value function needs to interact with the auction mechanism to reflect the value of the client through the price and support to select a set of suitable clients.
    
%     \myparagraph{C3}  \textit{Collecting the statistic of client's data might leak users' sensitive information}: In order to compute the value of the clients, the central server needs to know the global data distribution across clients and then selects a group of clients based the distribution while balancing the aforementioned metrics. However, the statistics regarding the quantity and the category distribution sent by each client are likely to disclose sensitive information about end users. For example, in the human activities recognition task, the distribution of activities may leak individual habits~\cite{qian2020orchestrating} and demoralize the participation of FL training. Thus, a privacy-preserving method can avoid revealing the category distribution of user data while obtaining aggregated information required by valuing function.

% \vspace{-2mm}
% \subsection{Our Contributions}

\myparagraph{Our Solution}
This paper presents \projecttitle, an incentivized  privacy-preserving client selection framework for FL.
We are targeting the setting of cross-silo FL across organizations such as healthcare~\cite{dayan2021federated} and finances~\cite{basu-etal-2021-privacy} where different organizations collaborate together in order to jointly train a global model. \projecttitle can collaborate between server and clients to collect the data statistics of the selected group of clients while ensuring their privacy and then price each selected client based on its data quality.
More specifically, to interact between clients and the server, 
we design a novel auction mechanism that accurately determines the maximum payment for each client and incentive them to bid their price based on their true cost.
To obtain clients' profiles (or data quality) for a given FL task, we design a value mechanism for evaluating the client data ahead of FL training by comprehensively considering the quantity and category distribution of the client data. Next, to avoid client privacy leakage during the profiling,
% Next, to obtain the quantity and category distribution of the client data (i.e., \textbf{C3}), 
we devise a novel \textit{additive secret sharing scheme} where the data distribution of a group of devices can be safely sent to the central server while the distribution of each device will not be disclosed. This mechanism enables the central server to acquire the global distribution of a group of devices -- particularly beneficial for the value function -- while preserving the sensitive information from the category distribution. 

\myparagraph{Results}
We compared \projecttitle with four state-of-the-art client selection baselines (RS, QBS, DICE and DDS, see Section \ref{sec:expsetup}) on two applications (image classification and human activity recognition) with three datasets (CIFAR10~\cite{krizhevsky2009learning}, CINIC10~\cite{darlow2018cinic} and DEAP~\cite{koelstra2011deap}). 
The experimental studies highlight that \projecttitle could significantly outperform other client selection baselines. 
Compared to other baselines, \projecttitle could improve the test accuracy up to 
47.50\%, 31.74\% and 29.21\% on CIFAR10, CINIC10 and DEAP, respectively. 
In addition, the convergence rate of \projecttitle is 
1.31 $\times$, 2.92 $\times$, 2.69 $\times$ and 2.08 $\times$ %\bin{2.83x and 3.68x} 
faster than four baselines respectively.   
\projecttitle can be integrated as a plug-in module to existing FL systems~\cite{liu2021fate,ziller2021pysyft,he2020fedml} and the source code will be made publish available.


\myparagraph{Research Contributions} This paper makes the following contributions:
\begin{enumerate}
    \item 
     To the best of our knowledge, \projecttitle is the first framework that addresses the desire for pre-training pricing for clients and effectively resolves the challenge of client selection for the server prior to FL training, which significantly enhances the incentive both for the server and clients (see Table~\ref{tab:comparsion}).
    
    \item We develop a new auction mechanism that interacts with both clients and servers to create a competitive environment that can result in a fair price for each client. 
    \item We propose a novel additive secret sharing scheme, which supports the evaluation of device data with the information of category distribution in a privacy-preserving manner.
\end{enumerate}

==> motivation-di.tex <==
\section{Federated Learning Data Market}
In this section, we first introduce a general data market that applies to many data trading scenarios.
Then, we consider transforming this market to a federated learning system and analyse the challenge in it.

\subsection{General Data Market}
The general data market consists of data providers, data consumers, and a market manager who operates the data market~\cite{jung2019privata}. 

\myparagraph{Data providers}: Data providers have a personalized dataset and wish to trade it for rewards. They will have a reserve price for their data and send it to the market manager.

\myparagraph{Data consumers}: Data consumers are businesses, researchers, or organizations that use big data to create products with business value.
Data consumers typically pay fees to collect data through the data market.

\myparagraph{Market manager}: The market manager is the key of the data market that aims to link data providers with consumers.
Sometimes his role is similar to that of an intermediary.

The interaction of them is shown in Figure \ref{fig:pipeline}.



%  \begin{figure}[t]
% \vspace{0mm}
%     \centering
%    \includegraphics[width=0.48\textwidth]{./figuresTex/figs/datamarket_1.pdf}
%     \vspace{-6mm}
%     \caption{Data market pipeline.}
%     \label{fig:pipeline}
%     \vspace{-6mm}
% \end{figure}





% In this section, we introduce the FL data market. To begin, we outline the primary components of the FL data market and present basic pipeline involving a typical FL task. Then, we delve into two crucial components for building an FL data market, namely the pricing mechanism and the privacy and security protocol. In addition, we emphasize the key challenge that must be addressed when designing above two components, respectively.

% \subsection{Key Components and Pipeline}
% \textbf{Key components.} In a typical federated learning data market, various entities play specific roles in the ecosystem. We present five key entities:

% \begin{enumerate}
%     \item Data providers: Data providers are organizations or individuals who own or have access to valuable datasets. They are willing to participate in the federated learning data market by contributing their data for model training. During a typical FL training, they are also named as FL clients, which could be IoT devices, mobile phone or institutions.
%     \item Data consumers: Data consumers are businesses, researchers, or organizations that create machine learning models or algorithms using data from the marketplace and deploy and utilize federated learning models for various applications after FL task. Data consumers typically pay fees to access the data.
%     \item FL platform: FL platforms serve as the technological backbone of the data market. These platforms enable data providers to securely share their data, while data consumers can train models on distributed data sources without direct access to the raw data. Federated learning platforms manage data aggregation, model updates, and ensure data privacy and security during the training.
%     % \item Pricing mechanism. In order to encourage data providers to participate in the federated learning data market, incentive mechanisms are often put in place. Particularly, it includes the pricing of financial rewards to motivate data providers to contribute their valuable data.
%     \item Pricing negotiation. In order to encourage data providers to participate in the federated learning data market, incentive mechanisms are often put in place. Particularly, it includes the pricing of financial rewards to motivate data providers to contribute their valuable data. However, data providers and data consumers sometimes don't know the value of the data. Therefore, the pricing negotiation helps to determine a reasonable price for data.
%     \item Privacy preserve. FL training employs privacy-preserving and secure techniques to train machine learning models without exposing raw data. Nevertheless, privacy and security protocols remain crucial for other components within an FL data market, e.g., the pricing process.
% \end{enumerate}

% These five entity components work together within the FL data market ecosystem to enable the secure, privacy-preserving exchange of data for machine learning model training with a privacy and security guarantee.

%  \label{subsec:pipeline}

%   \begin{figure}[t]
%  \vspace{0mm}
%      \centering
%     \includegraphics[width=0.48\textwidth]{./figuresTex/figs/datamarket.pdf}
%      \vspace{-6mm}
%      \caption{Data market pipeline.}
%      \label{fig:pipeline}
%      \vspace{-6mm}
%  \end{figure}
 
%  \textbf{Pipeline.}
%  A typical FL data market consists of four phases as shown in Figure~\ref{fig:pipeline}: 
%  \circled{1} \textit{Task Publication}: The data consumer (server) announces to all data providers (clients) with data requirements and budget of the anticipated FL task. 
%  \circled{2} \textit{Data Supply}: The data providers collect and select data according to the FL task requirements.
%  \circled{3} \textit{Data Evaluation}: After selecting the data, data providers need to know the value of their data. In FL data market, the data consumer is simultaneously responsible for evaluating the data. Therefore, the data providers share their data for evaluation through a privacy and security protocol.
%  \circled{4} \textit{Decision and Payment}: When data providers know the value of their data, they make a decision whether or not to participate. Then the data consumer negotiates the payment with the remaining data providers taking into account the value of data and the budget. Finally, the data consumer and data providers jointly determine the payment and winners.  
%  % A typical FL task consists of four phases as shown in Figure~\ref{fig:pipeline}~\cite{deng2021auction}: 
%  % \circled{1} \textit{Task Publication}: The central server announces to all registered clients with metadata of the anticipate FL task, including essential information regarding the topic of the task, the type of data recruited, and the eligibility of participants~\cite{hu2020trading,bonawitz2019towards}. 
%  % \circled{2} \textit{Client Selection}: It is impractical to allow all clients to participate in the task considering the limited budget of the central server, which places a demand on selecting high-quality clients allocating valuable payments~\cite{yu2020sustainable}.
%  % The clients interested in participating in the task are required to upload statistics (e.g. quantity and distribution of categories) of their own data for client selection in the server~\cite{nishio2019client}.
%  % \circled{3} \textit{Training}: All participants and the central server collaboratively train a global model using various FL aggregation algorithms (e.g. FedAvg~\cite{mcmahan2017communication}). 
%  % \circled{4} \textit{Reporting and Validation}: After each training round, including the end of the entire FL training process, participants report their updates (i.e. the updated weights of the model) and summaries of training (e.g. time consumption) to the central server. The central server conducts client validation and generates training logs for future reference. 

% \subsection{Pricing Negotiation}
% % Sometimes the data consumer is unable to determine the precise contribution of data from data providers before training. Thus, it is difficult for the data consumer to set the payment for the data. 
% % Meanwhile, the data providers don't know the value of their data.

% % \textbf{The Importance of Pre-training pricing.} 
% In most federated learning, client selection and payment determination are often dependent on contributions from training which needs all clients to participate FL training~\cite{liu2020fedcoin,wang2019measure,song2019profit,zeng2021comprehensive,zhan2021survey}. That wastes the computation and communication resources of unselected clients and will reduce clients' motivation to participate FL task.
% Selecting and pricing clients before training can not only save cost of computation and communication but also incentivise clients to join FL task because the clients who are not selected can exit the FL task before training begins and the selected clients can predict rewards.

% However, pricing before training makes it difficult for the server to access the contribution of data. Meanwhile, the clients are unable to evaluate the value of data in FL task. It is needed to formulate a pricing negotiation mechanism to determine a reasonable price for server and clients. 
% An auction is a great way to negotiate prices when data consumers and data providers are both unaware of the value of data.

% \myparagraph{Challenge 1} However, how to determine the initial price of data and the winner of the auction is the first challenge for us. Since data providers don't know the value of the data, it is difficult for clients to determine the bid for the auction. 
% For the server, selecting winners of the auction without the contribution and value of the data is difficult.

% \myparagraph{Solution} To solve the challenge proposed above, we consider formulating a pricing mechanism which first evaluates the data of the clients based on the evaluation function formulated by the server. Then pricing each client based on the result of evaluation, clients determine whether or not to participate in this task according to the price. Finally, clients send their bids to the server and the server combines the price and bid to select the winners and the payment for them.

% % In practice, a pricing mechanism is essential to motivate data providers to join a FL data market~\cite{zhan2021survey,zeng2021comprehensive,kairouz2021advances}.

% % From the perspective of data value, the task publisher in FL needs to compensate the clients for the value of the training data they provide. In addition, FL requires significant resource consumption, including computation power and bandwidth, which can be an undeniably cost for clients. Thus, voluntary collaboration in FL is normally impractical~\cite{LUO2019601}. 

% % The existing works on the FL incentive mechanism mainly focus on valuing contributions~\cite{liu2020fedcoin,wang2019measure,song2019profit,zeng2021comprehensive,zhan2021survey} of each individual client during or after the training phase, which leads to the negative outcomes:
% % 1) The contribution of users can only be evaluated after their participation in the FL training, lacking early estimation.
% % 2) More importantly, clients may be hesitant to participate in the training process if they do not see any tangible rewards for their efforts.

% % Compared to post-training incentives, pre-training incentives show merits both from the perspectives of clients and the server:
% % (1) From the perspective of the client, by offering predictable rewards before training, incentives can strongly motivate more clients to submit an application for the FL task and encourages clients to contribute high-quality and diversified data before training, ultimately leading to better training performance.
% % (2) Pre-training incentive mechanism is also necessary for the FL publisher (the server) since it provides an opportunity for estimating the value of client data, enabling more effective client selection and cost reduction of budget.

% % \myparagraph{C1} \textit{Designing an effective pricing mechanism to reach an optimal bidding price presents a significant challenge.}
% %      A key component of pre-training incentives is the pricing mechanism. An effective pricing mechanism should automatically make the clients and server reach a price consensus. There are two main difficulties in this process: first, clients tend to unrealistically pursue maximum returns if there is no limit on their bid; second, even if a client is rational, it is often impractical for them to accurately assess their maximum payment. To address this challenge, an effective pricing mechanism should be implemented, where the server provides well-designed rules for all rational clients to follow. This would enable them to automatically achieve the maximum reward they deserve based on the value they provided. However, designing an incentive mechanism that achieves this goal is challenging.
     
% % \subsection{Privacy and Security Protocol} 
% \subsection{Privacy Preserve}
% In pricing negotiation, the server formulates the evaluation function to evaluate data from clients. The data evaluation will involve the privacy of clients which is serious for FL. 


% \myparagraph{Threat model} The following threat model is prevalent in FL. 
% Each client and server is considered semi-honest, which means they are honest but curious. The client will execute the protocol honestly but try to learn sensitive information about other clients. Meanwhile, the server tries to infer sensitive information from the messages updated by clients.

% How to evaluate data 



% % How to profile the data in a privacy way which align with the core idea of federated learning that keep the raw data locally on clients.
 
% % \myparagraph{C2} \textit{Valuing clients under privacy constraints in advance of FL training is difficult.} 
% % The evaluation of client data is challenging since it is hard to precisely quantify the quality of data. 
% % When assessing high-quality clients, data quantity and distribution are important factors to consider.
% % However, solely relying on individual client evaluations does not effectively capture the impact of client interaction during training. 
% % Additionally, there is a lack of heuristic guidelines for designing data evaluation functions that consider both global and local data distribution.   
% % Further, during the evaluation process, the central server needs to access the data distribution of clients and then select a group of clients based on the distribution.
% % It is difficult to preserve sensitive information about end users when collecting such statistics regarding quantity and category distribution.





==> motivation.tex <==
\section{Motivation and Design Principles of \projecttitle}


In this section, we motivate the design principles of \projecttitle. Firstly, we introduce the basic pipeline of a FL tasks. Then, we discuss the importance of pre-training incentive for both the client and server. In addition, we highlight two challenges for designing an effective pre-training incentive mechanism. Finally, to solve the above challenges, we propose respective principles which serve as the main driving force behind the design of \projecttitle.


 \begin{figure}[t]
 \vspace{-3mm}
     \centering
    \includegraphics[width=0.35\textwidth]{./figuresTex/figs/big system.pdf}
     \vspace{-3mm}
     %\caption{The Pipeline of Federated Learning Task}
     \caption{The pipeline of federated learning task}
     \label{fig:pipeline}
     \vspace{-6mm}
 \end{figure}

 \subsection{The Pipeline of FL Task}
 \label{subsec:pipeline}
 
 FL task typically consists of four phases as shown in Figure~\ref{fig:pipeline}~\cite{deng2021auction}: 
 \circled{1} \textit{Task Publication}: The central server announces to all registered clients with metadata of the anticipate FL task, including essential information regarding the topic of the task, the type of data recruited, and the eligibility of participants~\cite{hu2020trading,bonawitz2019towards}. 
 \circled{2} \textit{Client Selection}: It is impractical to allow all clients to participate in the task considering the limited budget of the central server, which places a demand on selecting high-quality clients allocating valuable payments~\cite{yu2020sustainable}.
 The clients interested in participating in the task are required to upload statistics (e.g. quantity and distribution of categories) of their own data for client selection in the server~\cite{nishio2019client}.
 \circled{3} \textit{Training}: All participants and the central server collaboratively train a global model using various FL aggregation algorithms (e.g. FedAvg~\cite{mcmahan2017communication}). 
 \circled{4} \textit{Reporting and Validation}: After each training round, including the end of the entire FL training process, participants report their updates (i.e. the updated weights of the model) and summaries of training (e.g. time consumption) to the central server. The central server conducts client validation and generates training logs for future reference. 

 \subsection{ Data Sharing Model in Federated Learning}


 \subsection{The Importance of Pre-training Incentives} 

 In practice, an incentive mechanism is essential to motivate clients to participate in the FL task~\cite{zhan2021survey,zeng2021comprehensive,kairouz2021advances}. 
 From the perspective of data value, the task publisher in FL needs to compensate the clients for the value of the training data they provide. In addition, FL requires significant resource consumption, including computation power and bandwidth, which can be an undeniably cost for clients. 
 Thus, voluntary collaboration in FL is normally impractical~\cite{LUO2019601}. 

 The existing works on the FL incentive mechanism mainly focus on valuing contributions~\cite{liu2020fedcoin,wang2019measure,song2019profit,zeng2021comprehensive,zhan2021survey} of each individual client during or after the training phase, which leads to the negative outcomes:
 1) The contribution of users can only be evaluated after their participation in the FL training, lacking early estimation.
 2) More importantly, clients may be hesitant to participate in the training process if they do not see any tangible rewards for their efforts.

Compared to post-training incentives, pre-training incentives show merits both from the perspectives of clients and the server:
 (1) From the perspective of the client, by offering predictable rewards before training, incentives can strongly motivate more clients to submit an application for the FL task and encourages clients to contribute high-quality and diversified data before training, ultimately leading to better training performance.
 (2) Pre-training incentive mechanism is also necessary for the FL publisher (the server) since it provides an opportunity for estimating the value of client data, enabling more effective client selection and cost reduction of budget.
 

\subsection{Key Challenges of Pre-training Incentives}
 Although pre-training incentives have significant advantages, developing a practical and robust pre-training incentive framework is challenging. We have identified the following two key challenges:

  \myparagraph{C1} \textit{Designing an effective pricing mechanism to reach an optimal bidding price presents a significant challenge.}
     A key component of pre-training incentives is the pricing mechanism. An effective pricing mechanism should automatically make the clients and server reach a price consensus. There are two main difficulties in this process: first, clients tend to unrealistically pursue maximum returns if there is no limit on their bid; second, even if a client is rational, it is often impractical for them to accurately assess their maximum payment. To address this challenge, an effective pricing mechanism should be implemented, where the server provides well-designed rules for all rational clients to follow. This would enable them to automatically achieve the maximum reward they deserve based on the value they provided. However, designing an incentive mechanism that achieves this goal is challenging.

   \myparagraph{C2} \textit{Valuing clients under privacy constraints in advance of FL training is difficult.} 
   The evaluation of client data is challenging since it is hard to precisely quantify the quality of data. 
   When assessing high-quality clients, data quantity and distribution are important factors to consider.
   However, solely relying on individual client evaluations does not effectively capture the impact of client interaction during training. 
   Additionally, there is a lack of heuristic guidelines for designing data evaluation functions that consider both global and local data distribution.   
   Further, during the evaluation process, the central server needs to access the data distribution of clients and then select a group of clients based on the distribution.
   It is difficult to preserve sensitive information about end users when collecting such statistics regarding quantity and category distribution.

\subsection{Design Principles of \projecttitle}


\myparagraph{Truthful Auction Mechanism}
To address \textbf{C1}, we design an auction mechanism to allow the clients and server to reach a price consensus. Considering that some clients may be selfish and will ask for a reward that much higher than their contributions. This dishonest behavior undermines the integrity of the auction process and can lead to the server failing to obtain the real market price for performing the FL task, causing an unfair outcome. To this end, our auction mechanism needs to have a property that should reach an optimal bidding price where each client’s reward is maximized with its true value. We define an auction mechanism with this property as a \textbf{truthful} mechanism where auction participants (i.e. clients) should be encouraged to truthfully reveal their valuations, meaning that it is always in their best interest to honestly state their bid. Concretely, an auction mechanism is truthful if it satisfies the following conditions~\cite{singer2010budget}:
\begin{enumerate}
    \item Each client is priced at the maximum payment they could get denoted as the critical price.
    \item Each client can only argue for a bid price less than the critical price provided by the server. Otherwise, it will automatically lose the auction procedures.
\end{enumerate}


\begin{figure}[t]
\vspace{-3mm}
\centering
    \subfloat[Data quantity]{
    \includegraphics[height=.18\textwidth]{./figuresTex/figs/Amountandacc.pdf}
    \label{fig:Amountandacc}}
    \subfloat[Data balance]{
    \includegraphics[height=.18\textwidth]{./figuresTex/figs/motivation_data.pdf}
    \label{fig:motivation_data}}
    %\subfloat[Free rider attack]{
    %\includegraphics[width=.28\textwidth,height=0.192\textwidth]{./figuresTex/figs/motivation_fake.pdf}
    %\label{fig:motivation_fake}}
    \vspace{-3mm}
    %\caption{The Impact of Data Quantity and Distribution for Training
    %an FL Training Task.}
     \caption{The impact of data quantity and distribution for training
     an FL training task.}
    \label{fig:dsads}
    \vspace{-3mm}
\end{figure}

\myparagraph{Heuristic Rules and Privacy Requirements for Client Evaluation}
\label{sec:finding}
To address \textbf{C2}, we propose two heuristic rules and privacy requirements for client evaluation. we experimentally investigate the impact of two factors of data, i.e. quantity and distribution, by following experiments where we trained a popular ResNet-56~\cite{he2016deep} model using CIFAR-10~\cite{krizhevsky2012imagenet} dataset in a classical FL setting~\cite{mcmahan2017communication}.

\textit{The value of the client should be positively correlated to the size of data with a diminishing trend of marginal accuracy.}
To investigate the impact of data quantity, we examine the test accuracy of global models that are trained upon different volumes of data.
%In practice, we obtain 100 global models trained with the data size equally varying from 100 to 10,000 on each client. 
%We report the accuracy and its changes ($\Delta Accuracy$) for every 1,000 incremental data. 
Figure~\ref{fig:Amountandacc} shows the curve of test accuracy against the volume of data and bars of $\Delta Accuracy$ for every 1,000 incremental data. 
From the results, we could observe that the test accuracy increases with the increase in the amount of training data. However, the $\Delta Accuracy$ decreases rapidly, indicating that the marginal contribution of data to the test accuracy is limited when the data size is large.
% \textbf{Data Imbalance}
%In particular, we build an FL test bed with 20 clients with the aforementioned different levels of data imbalance and keep the number of total data among all clients the same (i.e. 32,000) to exclude the impact of the data size. We report the test accuracy of the FL training under the above setting to verify the impact of data imbalance.

\textit{The evaluation should encourage achieving a global balance across all classes.}
To evaluate the impact of data distribution, we compare the model accuracy under three distributions. 
(i) The data distributions are balanced across classes both locally for each client and globally for the server, namely \textit{local balance and global balance}. 
(ii) The data distribution is imbalanced locally but balanced globally, namely \textit{local imbalance and global balance}. 
(iii) The data distributions are both locally and globally imbalanced, namely \textit{local imbalance and global imbalance}.
Figure~\ref{fig:motivation_data} shows that the data imbalance significantly deteriorates the learning performance of FL training. 
%For instance, when the FL model is trained with \textit{local imbalance and global imbalance} setting, the final accuracy  drops dramatically from 87\% to 74\% when compared with the FL model trained with balanced data. 
However, when the global data is balanced while the local data is still imbalanced (the green curve in Figure~\ref{fig:motivation_data}), the accuracy degradation for FL training is much milder; 
%there is merely a 1\% accuracy loss lower than the ideal balance situation. 
In the practical scenario, the data distribution of local data is determined by the characteristics of end users, and hence cannot be controlled by the central server. Fortunately, the global distribution could be adjusted in the client evaluation process to mitigate the issue of local data imbalance.

\textit{When aggregating global distribution, it is significant that it can not expose the individual data distribution of each client.}
A privacy-preserving data evaluation method should be implemented to protect the privacy of the statistical information of clients. The server needs to learn about the global distribution through an encrypted approach, which means avoiding revealing the category distribution of the user's data. In particular, when the server evaluates the value of client data and aggregates the global data distribution, the data distribution of each client should not be known to the server.


==> soc.tex <==
\newpage
\section*{Summary of Changes}
\textbf{Title: \projecttitle: Enabling Privacy-preserved Pre-training Data Pricing for Federated Learning\\
Previous Submission Link: \\
https://openreview.net/forum?id=Bdj30CyxS8}\\
\\
% We would like to thank all the reviewers and the program chair for their time and constructive feedback on our previous submission. We have substantially revised the manuscript and provided a summary of the changes. Below, we outline our revisions based on the comments from the program chair and the reviewers.
We would like to thank all the reviewers and the PC for their constructive feedback to help us improve the quality of this paper. We have revised the manuscript substantially with new content as summarized below. Including the Appendix, the manuscript is now 15 pages long. We hope the extensive evaluation and comprehension would address all the reviewers' comments. 

\myparagraph{Primary revisions in response to PC comments} \\

C1: \textit{In some scenarios, especially in unbalanced data distribution, the accuracy of \projecttitle is not the best.}\\
R1: Across all 57 tested distributions, \projecttitle achieves the highest accuracy in 44 distributions (77\%). In terms of the most imbalanced distributions (D4, D5, and D6), \projecttitle achieves the highest accuracy in 22 out of 27 test distributions (81\%). We believe that the above statistical results can address the PC's concerns; therefore, we have explicitly included this analysis in lines 780-785 of Section \ref{sec:CSE}.

C2: \textit{It will be great if the method can be tested in the real-world FL data markets, or at least some discussion on the issues involving real-world deployment of the proposed method.}\\
R2: We have added a discussion section to address two key challenges when deploying our framework in FL data markets: the dynamics of FL data markets and malicious client attacks. Additionally, we provide potential solutions to mitigate these issues, which can be seamlessly integrated into our framework. It is important to note that we do not focus on these challenges in the design of our framework, as simple modifications or existing solutions can effectively address them, thereby minimizing their impact on our core contributions.

C3: \textit{The analysis and experimental results can be strengthened by adding some more recent works, some baselines are outdated.}\\
R3: We have added a comparison of \projecttitle to recent works from 2023-2024, such as martFL~\cite{li2023martfl}, DEVELOP~\cite{sun2022profit}, and SARDA~\cite{sun2024socially} in Table~\ref{tab:comparsion} of Appendix~\ref{related_work_table}. Further analysis of these recent works~\cite{mao2024game,sun2024socially,li2024performance,Ren2024noniidauction} can be found in the Related Work section. Additionally, when selecting baselines for our experiments, we explicitly explained the rationale behind our choices in lines 694–734.

\myparagraph{Other revisions based on reviewer comments} \\

C4: \textit{Motivation for pre-training pricing}\\
R4: To further underscore our motivation for pre-training pricing to encourage FL participation, we have included an empirical survey,  as shown in Appendix \ref{appendix:survey}, to bolster our argument.
The survey is about the pricing mechanism in FL influences users’ participation willingness, and we collected a total of 53 questionnaires
on five questions.

C5: \textit{Further clarification is needed for the choice of the logarithmic function for $f(\cdot)$ in equation \ref{eq:quantity_coe}.}\\
R5: To address this point, we explicitly introduced the reasons for choosing \(f(\cdot)\) in lines 306 to 311 of Section \ref{subsec:first-round}. Further details are explained in Appendix~\ref{sec:sen_analysis}, where both theoretical supports and empirical evidences are provided for the selection of \(f(\cdot)\) to model the relationship between data volume and accuracy. Additionally, we redesigned the experimental candidate functions from the family of logarithmic functions.

C6: \textit{Results of test accuracy vs. rounds.}\\
R6: We have added the results of each round's test accuracy, as shown in Figure~\ref{fig:my_convergence}, along with a corresponding analysis of convergence speed.


C7: \textit{Restructuring certain sections and revising typos}\\
R7: We moved the related work section to follow the introduction and added the convergence speed paragraph, previously in the Appendix, to the evaluation section. Additionally, we carefully revised the paper to correct the typos noted by the reviewers, as well as any others we identified.

==> system_Implementation.tex <==
% \section{\projecttitle Implementation}
% \label{sec:implementation}
% We have implemented \projecttitle as a Python library, which contains not only the class for traditional FL process but also the three key classes for \projecttitle, i.e. data evaluation class, ASS class and anti-fraud class. We packed and presented \projecttitle into a Docker~\footnote{https://www.docker.com} container for the easy deployment of cross-silo clients and the central server. The container of \projecttitle includes the training engine (e.g. Pytorch~\footnote{https://pytorch.org} and Tensorflow~\footnote{https://tensorflow.org}), the communication backend(e.g. gRPC~\footnote{https://grpc.io}) and functional classes of \projecttitle.

\begin{figure}[t]
\centering
    \includegraphics[width=0.3\textwidth,height=0.4\textwidth]{./figuresTex/figs/Implementation.pdf}
    \caption{Implementation of ASS-GAD under PS Architecture}
    \label{fig:Imp_ASS_GAD}
    \vspace{-4mm}
\end{figure}

\subsection{Implementing ASS-GAD in Parameter Server Architecture}
\label{sec:assgadps}
The vanilla implementation of ASS requires a peer-to-peer connection between all the clients at the \textbf{exchange} phase, which is a high assumption under the FL training paradigm.
If we apply ASS-GAD to Parameter Server (PS) which is the most representative computational architecture for FL, the central server will directly obtain clients' distributions.
% In reality, it is infeasible that all clients establish connections between each other, especially when there are large number of clients in the client pool. 
To overcome this problem, in \projecttitle we have designed a privacy-preserving approach for the implementation of ASS-GAD with a PS architecture as shown in Figure~\ref{fig:Imp_ASS_GAD}.
 
Our implementation is based on cryptography with public and private keys.
For each client, a pair of public and private keys are generated with OpenSSL\footnote{https://www.openssl.org/} at each edge node.
The public keys are sent to the server and re-transmitted to all other clients.
Next, during the \textbf{exchange} phase, each client encrypts divided class distributions with corresponding public keys and sends them to other clients via the server.
In the \textbf{local fusion} phase, the clients decode the received information with private keys to obtain the data distributions sent from other clients. 
Finally, the \textbf{global fusion} is implemented with all aggregated data distributions.  
The cryptography techniques are effective in securing the transmitted data distribution, not directly seen by the server side.



% \zy{add a simple figure to show how the key exchange works.}

% \zy{add the something about how to implement the key exchanging in PS }

% At the initialization of a FL task, each client needs to pull the image from the central server containing the metadata and initialization steps of the FL task. The metadata and initialization information are stored as a configuration file (e.g. PyYAML~\footnote{https://pyyaml.org}) in the Docker image. When each client launch the image, the initialization code will be started up for building the connection links as a fully peer-to-peer network for communication between clients and the central server for the execution of data distribution sharing scheme (\ref{alg:ASSGAD}). After that, The four phases of FL task shown in \ref{fig:pipeline} will be run using the modules in the \projecttitle docker container.

==> system_Incentive.tex <==


\subsection{Client Profiling with Data Score Function}
\label{sec:data_evaluation}

% Based on motivation experiments, we define the following goals for selecting high-quality clients.

% \myparagraph{Goal 1} \emph{All selected clients should contain sufficient data, and the number of data among all classes is similar, i.e., the data distribution is uniform for all classes across all selected clients.}

% Obviously, this is an ideal situation in FL, but in most cases is not possible to be achieved. 
% Thus, the following goal is defined as a desired goal for client selection.

% \myparagraph{Goal 2} \emph{The selected clients should contain 
% sufficient data and should contain data for all classes. The overall data distribution for all selected clients is uniform.}

% Understandably, goal 2 is a relaxed condition as compared to goal 1.
% In order to achieve goal 2, proper data evaluation conditions and client selection mechanisms are designed as follows. 

% \zy{In order to achieve \textit{goal 2}, \projecttitle defines a data score function $\mathcal{U}$ that considers two factors in granularity: 1) \textit{Data Quantity}; 2) \textit{Data Rarity}.}

% Let $n^{c}$ denotes the total number of data for class $c$, i.e., $ N = [n^{1}, n^{2} \\... n^{C} ]$ and $\sum_{c=1}^{C} n^{c} = n$, the data score function $\mathcal{U}$ is defined as follows.
% \begin{equation}
% \mathcal{U} (N, n_e^c) = \sum_{c=1}^{C} \theta_{c} (N) \cdot \phi(n_{e}^{c})
% \label{eq:data_evaluation}
% \end{equation}

Let $n^{c}$ denotes the total number of data for class $c$, i.e. $ N = [n^{1}, n^{2} \\... n^{C} ]$ and $\sum_{c=1}^{C} n^{c} = n$, we sums up data score of each class $c$ as client's data score. The class data score function $\mathcal{V}$ is defined as follows.
\begin{equation}    
    \mathcal{V}(N,n_e^c)=\theta_{c} (N) \cdot \phi(n_{e}^{c})
\end{equation}
and the client's data score function $\mathcal{U}$ is defined as
\begin{equation}
    \mathcal{U} (N, n_e^c) = \sum_{c=1}^{C} \mathcal{V}(N,n_e^c)
\end{equation}

Data score is affected by two things: data quantity and data rarity. Then the class data score function $\mathcal{V} (N, n_e^c)$ considering two coefficients:
1) data quantity coefficient $\phi(n_{e}^{c})$, on the other hand, is a specific coefficient that gives the value based on data samples $n_e^{c}$ belonging to class $c$.
2) data rarity coefficient $\theta_{c} (N)$ is a generic coefficient with respect to global data distribution $N$ and calculates the rarity of each class $c$ from $N$.  


% where $\theta_{c}$ is data rarity coefficient that evaluates the extend of the data rarity for each class $c$. $\phi(n_{e}^{c})$ is data quantity coefficient that measures the data quantity on each client. 

% $\mathcal{U} (N, n_e^c)$ sums up the value score of individual data samples across all classes $\theta_{c}$, with each class $c$ considering two coefficients: 
% 1) data rarity coefficient $\theta_{c} (N)$ is a generic coefficient with respect to global data distribution $N$ and calculates the rarity of each class $c$ from $N$.
% 2) data quantity coefficient $\phi(n_{e}^{c})$, on the other hand, is a client-specific coefficient that gives the value based on data samples $n_{e}^{c}$ belonging to class $c$ on each client $e$. 

\myparagraph{Profiling Process}
In our client profiler, we first aggregate and get global data distribution $N$ with carefully designed heuristics (Section~\ref{sec:ass}).
Then, both $N$ and $\mathcal{U} (N, n_e^c)$ will be sent to the clients, where the clients compute the data score $u_e$ with $n_e^c$ and $N$ altogether.
Finally, all $[u_e, \forall e \in E]$ will be sent back to the server for calculation of the server-side utility function (Equation~\ref{eq:utilityfunction} in Section~\ref{sec:auctiondefinition}) of each client $e$.
The clients that contain rarer class data and sufficient data volume will have higher scores and are regarded as high-quality clients. 
The following illustrates the details of two coefficients.

\subsubsection{Data Quantity Coefficient}

Our observation of the effect of model accuracy with the amount of data shows that the effect of data volume on accuracy is progressively reduced, thus we model this effect as a function of the integral of $-lnx$ over the interval [0-1].
The quantity coefficient for individual class $c$ is defined as: 
\begin{equation}
    \phi(n_{e}^{c}) = \int_{0}^{r_e^c} -lnx dx
\label{eq:quantity_coe}
\end{equation}

We set $r_e^c$ as the upper limit of integration for the function, and $r_e^c$ is a normalized value of $n_e^c$ to set all $\phi(n_e^c)$ to the same scale. 
We assume that when $n_{e}^{c} \geq n / (E, C)$, any class that contains more than the average number of data will not receive a further reward. Thus we define the max value of $r_e^c$ as 1. When the data volume of class $c$ on client $e$ is greater than $\frac{n}{E\cdot C}$, $r_e^c=1$.
\begin{equation}
    % r_e^c = \min \{ \frac{n_{e}^{c}}{n/ (E \cdot C)} , 1\} 
r_e^c =\left\{\begin{matrix}
\frac{n_{e}^{c}}{n/ (E \cdot C)}, n_e^c<\frac{n}{E\cdot C}\\ 
1,n_e^c\geq\frac{n}{E\cdot C}
\end{matrix}\right.
\end{equation}


% On client $e$, the quantity coefficient for individual class $c$ is defined by $\phi(n_{e}^{c})$:
% % \begin{equation}
% % \begin{split}
% %     \phi(n_{e}^{c}) &= \int_{0}^{r(e,c)} f(x) dx \\
% %     r(e,c)          &= \min \{ \frac{n_{e}^{c}}{n/ (E \cdot C)} , 1\} 
% % \end{split}
% % \label{eq:quantity_coe}
% % \end{equation}
% \begin{equation}
% % \begin{split}
%     \phi(n_{e}^{c}) = \int_{0}^{r_e^c} f(x) dx
% %     r(e,c)          &= \min \{ \frac{n_{e}^{c}}{n/ (E \cdot C)} , 1\} 
% % \end{split}
% \label{eq:quantity_coe}
% \end{equation}

% $f(x)$ represents the value of each individual data sample, and $r_e^c$ indicates the data volume of class $c$ on client $e$.
% With $\phi(n_{e}^{c})$, we sum up the value of individual data samples in granularity. 


% The choice of sample value function $f(x)$ requires monotonically decreasing properties in the interval 0 to 1, indicating that the contribution decreases as the number of data increases. 
% In \projecttitle, we set $f(x) = - ln(x)$, which empirically works best in our experiments.
% We also report the performance of different candidate functions as detailed in Section~\ref{sec:sen_analysis}.
% We also add certain constraints to $r_e^c$ as well.
% \begin{equation}
% % \begin{split}
%     % \phi(n_{e}^{c}) &= \int_{0}^{r(e,c)} f(x) dx \\
%     r_e^c = \min \{ \frac{n_{e}^{c}}{n/ (E \cdot C)} , 1\} 
% % \end{split}
% % \label{eq:quantity_coe}
% \end{equation}

% Assume $n_{e}^{c}$ is the number of data for class $c$ in local client $e$, there are $E$ clients and $C$ classes in total.
% We normalize $n_{e}^{c}$ to $r_{e}^{c}$  $\in [0,1]$ such that all $\phi(n_{e}^{c})$ are set to the same scale.
% We also set the maximum value of $r_e^c$ to 1, such that when $n_{e}^{c} \geq n / (E, C)$, any class that contains more than the average number of data will not receive a further reward.
% This helps prioritizes clients with reasonable amounts of data and containing data samples in all classes, in contrast to clients containing large volumes of data but missing samples in certain classes.

\myparagraph{The importance of modeling Data Quantity in Granularity}
Figure~\ref{fig:Amountandacc} shows that the data quantity is highly correlated with the final training accuracy.
When few data are available during the training process, a slight increase in data quantity could significantly improve the training accuracy.
As more data are added to the training set, the newly added data contribute less to performance gain. 
Thus we model this non-linear relation between the data quantity and the training accuracy with data quantity coefficient $\phi(n_{e}^{c})$ (i.e., Equation~\ref{eq:quantity_coe}) to denote the importance of each individual data sample. 

\subsubsection{Data Rarity Coefficient}
The data quantity coefficient assumes equality importance for samples across different classes. However, valuing more rare classes helps to improve the uniformity of final global data distribution. 
The rarity of the class $c$ data is defined by $\theta_{c}$:
\begin{equation}
 \theta_{c} (N) =  1 - n^{c} / n
\end{equation}
$n^{c}$ is the total number of data for class $c$ and $n$ is the total number of data in $N$.
We use min-max normalization \cite{friedman2019assessment} to normalize $\theta_{c}(N)$ for $\forall   n^{c} \in N$ and rescale it such that $ \theta_{c}(N) \in [\min\{{N}\}, \max{\{N}\}]$.
We also validate the necessity of $\theta_{c}(N)$ in Section \ref{sec:sen_analysis} and Figure~\ref{fig:test_theta}.

% 2) \textit{Data Rarity:}
% From Figure~\ref{fig:motivation_data}, we notice the importance of a globally balanced dataset on the final performance of model training.
% However, in a real FL client pool, it is unlikely that the data are evenly distributed, thus the rare data samples are less likely to be selected to join the training.
% In order to select these rarer data to join the training, we need to design a data rarity coefficient $\theta_{c}$ based on global class distribution and gives higher value to globally rarer data. 

==> system_goal.tex <==
\bin{
\subsection{Design Goal}

Ideally, in order for FL training to achieve the best performance, the selected clients should achieve the following goal:

\myparagraph{Goal 1} \emph{All selected clients should contain sufficient data, and the number of data among all classes is similar, i.e., the data distribution is uniform for all classes across all selected clients.}

Obviously, this is an ideal assumption in FL: globally and locally balanced data across all devices, in most cases, is not possible to be achieved. 
A more realistic goal is defined as follows for client selection.

\myparagraph{Goal 2} \emph{The selected clients should contain sufficient data and should contain data for all classes. 
The overall data distribution for all selected clients is uniform.}

Goal 2 is closely related to our findings in Figure~\ref{fig:dsads}: 
1) Figure~\ref{fig:Amountandacc} presents the importance of at least a few examples for each class during training, clients with complete data samples in each class are regarded as high-quality clients;
2) and in Figure~\ref{fig:motivation_data}, the \textit{local imbalanced \& global balanced} data distribution can achieve slightly inferior performance compared to the uniform data distribution presented in Goal 1. 
Understandably, goal 2 is a relaxed but realistic condition as compared to goal 1.

With goal 2 in mind, \projecttitle has made two efforts to achieve this goal.

\myparagraph{Effort 1}
We design a novel data score function to realize our goal of selecting high-quality clients and generating globally balanced data distribution.
In response to C2, our data score function values local data samples in granularity while emphasizing more on globally scarce data samples. 
In contrast to previous work on valuing data samples, we are the only work that considers global data distributions, thus are better at selecting clients with real valuable data samples.  (Section.~\ref{sec:data_evaluation})

\myparagraph{Effort 2}
To realize \textit{Effort 1} requires the knowledge of global data distributions. 
In response to C3, we design a privacy-preserving approach for collecting data statistics and parameterising the data score function.
Considering that the clients can not communicate with each other in FL, we novely design an encrypted additive secret-sharing protocol for securely aggregating data distributions (Section.~\ref{sec:ass}). 


}
